Benchmarking World-Model Learning with Environment-Level Queries

World models are central to building AI agents capable of flexible reasoning and planning. Yet current evaluations (i) test only properties measurable from observed interactions, such as next-frame prediction or task return, and (ii) do not test whether a learned model supports diverse queries about the environment. In contrast, humans build $\textit{general-purpose}$ models that can answer many different questions about an environment$\unicode{x2014}$including questions that require understanding global structure and counterfactual consequences. We propose $\textit{WorldTest}$: a protocol for evaluating whether agents learn models that support multiple $\textit{environment-level queries}\unicode{x2014}$questions whose answers depend on properties of the full environment, not just observed trajectories. Individually, these queries can target properties (e.g., reachability or the effects of interventions) that no single rollout distribution determines. Collectively, they assess model generality across query types. We instantiate WorldTest as $\textit{AutumnBench}$, a benchmark of 43 interactive grid-world environments and 129 tasks across three query families for both humans and learning agents. Experiments with 517 human participants and five frontier models show that humans substantially outperform these models, a gap we attribute to differences in exploration and belief updating. AutumnBench provides a framework for evaluating world-model learning in grid-world environments with environment-level queries, and WorldTest provides a template for extending such evaluations to richer domains.

==> main-aux.tex <==
\begin{filecontents}
{main.aux}
\relax 
\providecommand\hyper@newdestlabel[2]{}
\providecommand\HyField@AuxAddToFields[1]{}
\providecommand\HyField@AuxAddToCoFields[2]{}
\providecommand\BKM@entry[2]{}
\BKM@entry{id=1,dest={73656374696F6E2E32},srcline={382}}{5C3337365C3337375C303030495C3030306E5C303030745C303030725C3030306F5C303030645C303030755C303030635C303030745C303030695C3030306F5C3030306E}
\citation{Weisberg2013}
\citation{LeCun2022APT}
\citation{brockman2016openai}
\citation{bongard,arc_paper}
\citation{discoveryworld}
\citation{kexin2021clevrer}
\providecommand\csxdef[2]{}
\@writefile{toc}{\providecommand\autonum@processReference[2]{}}
\@writefile{lof}{\providecommand\autonum@processReference[2]{}}
\@writefile{toc}{\contentsline {section}{\numberline {1}Introduction}{1}{section.2}\protected@file@percent }
\newlabel{sec:introduction}{{1}{1}{}{section.2}{}}
\newlabel{sec:introduction@cref}{{[section][1][]1}{[1][1][]1}{}{}{}}
\@writefile{toc}{\contentsline {paragraph}{Benchmarking World-Model Learning with Environment\Hyphdash  Level Queries}{1}{Item.6}\protected@file@percent }
\@writefile{lof}{\contentsline {figure}{\numberline {1}{\ignorespaces Overview of the WorldTest\xspace  framework and the AutumnBench instantiation. Agents first interact with an environment without external rewards to build a world model, then act in a derived challenge environment for evaluation. Top-left box shows the 9 example AutumnBench environments. Yellow notes in the middle explain the key UI elements in the human interface of AutumnBench. }}{2}{figure.caption.3}\protected@file@percent }
\providecommand*\caption@xref[2]{\@setref\relax\@undefined{#1}}
\newlabel{fig:pipeline_overview}{{1}{2}{Overview of the \wmla framework and the AutumnBench instantiation. Agents first interact with an environment without external rewards to build a world model, then act in a derived challenge environment for evaluation. Top-left box shows the 9 example AutumnBench environments. Yellow notes in the middle explain the key UI elements in the human interface of AutumnBench}{figure.caption.3}{}}
\newlabel{fig:pipeline_overview@cref}{{[figure][1][]1}{[1][1][]2}{}{}{}}
\@writefile{toc}{\contentsline {paragraph}{Our Approach}{2}{Item.9}\protected@file@percent }
\citation{lance2025assessing}
\citation{vbench}
\citation{svib}
\citation{kexin2021clevrer}
\citation{acre}
\citation{raven}
\citation{pgm}
\citation{bongard}
\citation{arc_paper}
\citation{puzzles}
\citation{procgen}
\citation{discoveryworld}
\citation{alchemy}
\citation{causalworld}
\citation{phyre}
\citation{nethack}
\citation{minihack}
\citation{bellemare2013arcade}
\citation{laskin2021urlbunsupervisedreinforcementlearning}
\BKM@entry{id=2,dest={73656374696F6E2E3137},srcline={823}}{5C3337365C3337375C303030525C303030655C3030306C5C303030615C303030745C303030655C303030645C3030305C3034305C303030575C3030306F5C303030725C3030306B5C30303073}
\citation{arc_paper,bongard,pgm,svib,acre,kexin2021clevrer}
\citation{bongard}
\citation{acre,kexin2021clevrer}
\citation{arc_paper}
\citation{movingmnist,bairrobotpushing}
\citation{discoveryworld}
\citation{kexin2021clevrer,girdhar2020cater,causalworld}
\citation{brockman2016openai,bellemare2013arcade,procgen,nethack,minihack,causalworld,alchemy,dmcsuite}
\citation{laskin2021urlbunsupervisedreinforcementlearning}
\citation{laskin2023ad}
\@writefile{toc}{\contentsline {paragraph}{Contributions}{3}{Item.15}\protected@file@percent }
\csxdef {autonum@sec:related-workReferenced}{}
\csxdef {autonum@sec:backgroundReferenced}{}
\csxdef {autonum@sec:wmla-and-benchReferenced}{}
\csxdef {autonum@sec:baseline-evaluations-and-analysisReferenced}{}
\csxdef {autonum@sec:conclusionReferenced}{}
\@writefile{toc}{\contentsline {section}{\numberline {2}Related Works}{3}{section.17}\protected@file@percent }
\newlabel{sec:related-work}{{2}{3}{}{section.17}{}}
\newlabel{sec:related-work@cref}{{[section][2][]2}{[1][3][]3}{}{}{}}
\csxdef {autonum@tab:benchmark_comparisonReferenced}{}
\BKM@entry{id=3,dest={73656374696F6E2E3138},srcline={857}}{5C3337365C3337375C303030425C303030615C303030635C3030306B5C303030675C303030725C3030306F5C303030755C3030306E5C30303064}
\citation{autumnsynth}
\BKM@entry{id=4,dest={73656374696F6E2E3139},srcline={892}}{5C3337365C3337375C303030545C303030685C303030655C3030306F5C303030725C303030655C303030745C303030695C303030635C303030615C3030306C5C3030305C3034305C303030465C303030725C303030615C3030306D5C303030655C303030775C3030306F5C303030725C3030306B5C3030305C3034305C303030615C3030306E5C303030645C3030305C3034305C303030425C303030655C3030306E5C303030635C303030685C3030306D5C303030615C303030725C3030306B}
\BKM@entry{id=5,dest={73756273656374696F6E2E3230},srcline={920}}{5C3337365C3337375C303030575C3030306F5C303030725C3030306C5C303030645C303030545C303030655C303030735C303030745C3030305C3034305C303030465C303030725C303030615C3030306D5C303030655C303030775C3030306F5C303030725C3030306B}
\@writefile{lot}{\contentsline {table}{\numberline {1}{\ignorespaces Comparison of benchmarks in the literature. MDP refers to Markov Decision Process, DET-POMDP refers to Deterministic-Partially Observable Markov Decision Process, and POMDP refers to Partially Observable Markov Decision Process. POMDP is the most general type of environment.}}{4}{table.caption.16}\protected@file@percent }
\newlabel{tab:benchmark_comparison}{{1}{4}{Comparison of benchmarks in the literature. MDP refers to Markov Decision Process, DET-POMDP refers to Deterministic-Partially Observable Markov Decision Process, and POMDP refers to Partially Observable Markov Decision Process. POMDP is the most general type of environment}{table.caption.16}{}}
\newlabel{tab:benchmark_comparison@cref}{{[table][1][]1}{[1][3][]4}{}{}{}}
\@writefile{toc}{\contentsline {section}{\numberline {3}Background}{4}{section.18}\protected@file@percent }
\newlabel{sec:background}{{3}{4}{}{section.18}{}}
\newlabel{sec:background@cref}{{[section][3][]3}{[1][4][]4}{}{}{}}
\@writefile{toc}{\contentsline {paragraph}{Partially Observable Markov Decision Processes (POMDPs).}{4}{section.18}\protected@file@percent }
\csxdef {autonum@fig:pipeline_overviewReferenced}{}
\@writefile{toc}{\contentsline {paragraph}{The Autumn Language.}{4}{section.18}\protected@file@percent }
\csxdef {autonum@sec:autumnReferenced}{}
\@writefile{toc}{\contentsline {section}{\numberline {4}Theoretical Framework and Benchmark}{4}{section.19}\protected@file@percent }
\newlabel{sec:wmla-and-bench}{{4}{4}{}{section.19}{}}
\newlabel{sec:wmla-and-bench@cref}{{[section][4][]4}{[1][4][]4}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.1}WorldTest\xspace  Framework}{4}{subsection.20}\protected@file@percent }
\@writefile{toc}{\contentsline {paragraph}{Intuition.}{4}{subsection.20}\protected@file@percent }
\BKM@entry{id=6,dest={73756273656374696F6E2E3239},srcline={1016}}{5C3337365C3337375C303030415C303030755C303030745C303030755C3030306D5C3030306E5C303030425C303030655C3030306E5C303030635C303030685C3030303A5C3030305C3034305C303030445C303030655C303030735C303030695C303030675C3030306E5C3030305C3034305C303030615C3030306E5C303030645C3030305C3034305C303030495C3030306D5C303030705C3030306C5C303030655C3030306D5C303030655C3030306E5C303030745C303030615C303030745C303030695C3030306F5C3030306E}
\citation{autumnsynth}
\citation{lance2025assessing}
\citation{bellemare2013arcade}
\citation{nim}
\newlabel{sec:formal-def}{{4.1}{5}{}{Item.22}{}}
\newlabel{sec:formal-def@cref}{{[subsection][1][4]4.1}{[1][5][]5}{}{}{}}
\@writefile{toc}{\contentsline {paragraph}{Formal Definition.}{5}{Item.22}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {4.2}AutumnBench: Design and Implementation}{5}{subsection.29}\protected@file@percent }
\@writefile{toc}{\contentsline {paragraph}{Interaction-Phase Environments.}{5}{Item.31}\protected@file@percent }
\csxdef {autonum@tab:program_statsReferenced}{}
\BKM@entry{id=7,dest={73656374696F6E2E3332},srcline={1083}}{5C3337365C3337375C303030425C303030615C303030735C303030655C3030306C5C303030695C3030306E5C303030655C3030305C3034305C303030455C303030765C303030615C3030306C5C303030755C303030615C303030745C303030695C3030306F5C3030306E5C303030735C3030305C3034305C303030615C3030306E5C303030645C3030305C3034305C303030415C3030306E5C303030615C3030306C5C303030795C303030735C303030695C30303073}
\citation{prolific}
\BKM@entry{id=8,dest={73756273656374696F6E2E3333},srcline={1109}}{5C3337365C3337375C303030455C303030765C303030615C3030306C5C303030755C303030615C303030745C303030695C3030306F5C3030306E5C3030305C3034305C303030535C303030655C303030745C303030755C30303070}
\BKM@entry{id=9,dest={73756273756273656374696F6E2E3334},srcline={1114}}{5C3337365C3337375C303030485C303030755C3030306D5C303030615C3030306E5C3030305C3034305C303030455C303030765C303030615C3030306C5C303030755C303030615C303030745C303030695C3030306F5C3030306E}
\citation{Muszyski2023}
\citation{reid2022softwareengineeringuserstudy,Douglas2023}
\BKM@entry{id=10,dest={73756273756273656374696F6E2E3336},srcline={1171}}{5C3337365C3337375C303030525C303030655C303030615C303030735C3030306F5C3030306E5C303030695C3030306E5C303030675C3030302D5C3030304D5C3030306F5C303030645C303030655C3030306C5C3030305C3034305C303030455C303030765C303030615C3030306C5C303030755C303030615C303030745C303030695C3030306F5C3030306E}
\csxdef {autonum@fig:pipeline_overviewReferenced}{}
\csxdef {autonum@sec:env_detailsReferenced}{}
\@writefile{toc}{\contentsline {paragraph}{Test-Phase Challenges.}{6}{Item.31}\protected@file@percent }
\csxdef {autonum@sec:formal-defReferenced}{}
\csxdef {autonum@sec:baseline-evaluations-and-analysisReferenced}{}
\csxdef {autonum@sec:challenge-formulationReferenced}{}
\@writefile{toc}{\contentsline {section}{\numberline {5}Baseline Evaluations and Analysis}{6}{section.32}\protected@file@percent }
\newlabel{sec:baseline-evaluations-and-analysis}{{5}{6}{}{section.32}{}}
\newlabel{sec:baseline-evaluations-and-analysis@cref}{{[section][5][]5}{[1][6][]6}{}{}{}}
\csxdef {autonum@sec:setupReferenced}{}
\csxdef {autonum@sec:autumn-simulator-agentReferenced}{}
\csxdef {autonum@sec:resultsReferenced}{}
\csxdef {autonum@sec:discussionReferenced}{}
\@writefile{toc}{\contentsline {subsection}{\numberline {5.1}Evaluation Setup}{6}{subsection.33}\protected@file@percent }
\newlabel{sec:setup}{{5.1}{6}{}{subsection.33}{}}
\newlabel{sec:setup@cref}{{[subsection][1][5]5.1}{[1][6][]6}{}{}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {5.1.1}Human Evaluation}{6}{subsubsection.34}\protected@file@percent }
\csxdef {autonum@sec:formal-defReferenced}{}
\csxdef {autonum@fig:pipeline_overviewReferenced}{}
\csxdef {autonum@sec:task-guiReferenced}{}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {5.1.2}Reasoning-Model Evaluation}{6}{subsubsection.36}\protected@file@percent }
\BKM@entry{id=11,dest={73756273656374696F6E2E3436},srcline={1233}}{5C3337365C3337375C303030525C303030655C303030735C303030755C3030306C5C303030745C30303073}
\BKM@entry{id=12,dest={73756273756273656374696F6E2E3437},srcline={1248}}{5C3337365C3337375C3030304F5C303030765C303030655C303030725C303030615C3030306C5C3030306C5C3030305C3034305C303030505C303030655C303030725C303030665C3030306F5C303030725C3030306D5C303030615C3030306E5C303030635C30303065}
\BKM@entry{id=13,dest={73756273756273656374696F6E2E3439},srcline={1272}}{5C3337365C3337375C303030455C303030785C303030705C3030306C5C3030306F5C303030725C303030615C303030745C303030695C3030306F5C3030306E5C3030305C3034305C303030505C303030615C303030745C303030745C303030655C303030725C3030306E5C30303073}
\newlabel{fig:stochastic_vs_det}{{3a}{7}{Score by Stochasticity}{figure.caption.35}{}}
\newlabel{fig:stochastic_vs_det@cref}{{[subfigure][1][3]3a}{[1][6][]7}{}{}{}}
\newlabel{sub@fig:stochastic_vs_det}{{a}{7}{Score by Stochasticity}{figure.caption.35}{}}
\newlabel{sub@fig:stochastic_vs_det@cref}{{[subfigure][1][3]3a}{[1][6][]7}{}{}{}}
\newlabel{fig:score_by_task_type}{{3b}{7}{Score by Task Type}{figure.caption.35}{}}
\newlabel{fig:score_by_task_type@cref}{{[subfigure][2][3]3b}{[1][6][]7}{}{}{}}
\newlabel{sub@fig:score_by_task_type}{{b}{7}{Score by Task Type}{figure.caption.35}{}}
\newlabel{sub@fig:score_by_task_type@cref}{{[subfigure][2][3]3b}{[1][6][]7}{}{}{}}
\newlabel{fig:score_by_env_violin}{{3c}{7}{Score}{figure.caption.35}{}}
\newlabel{fig:score_by_env_violin@cref}{{[subfigure][3][3]3c}{[1][6][]7}{}{}{}}
\newlabel{sub@fig:score_by_env_violin}{{c}{7}{Score}{figure.caption.35}{}}
\newlabel{sub@fig:score_by_env_violin@cref}{{[subfigure][3][3]3c}{[1][6][]7}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {3}{\ignorespaces Aggregate scores over all AutumnBench problems. (a) Reasoning models perform better in stochastic environments than in deterministic ones, while humans perform consistently across both. (b) Humans outperform reasoning models across the three task families: CD, MFP, and planning. (c) Environment-wise score distributions per agent across the 129 AutumnBench problems.}}{7}{figure.caption.35}\protected@file@percent }
\csxdef {autonum@sec:formal-defReferenced}{}
\csxdef {autonum@fig:prompt_exampleReferenced}{}
\@writefile{lof}{\contentsline {figure}{\numberline {2}{\ignorespaces Textual representation of the top grid in the ``interaction phase'' of \autonum@processReference {autonum@referenceCrefOld}{forcsvlist}{fig:pipeline_overview}.}}{7}{figure.caption.37}\protected@file@percent }
\csxdef {autonum@fig:pipeline_overviewReferenced}{}
\newlabel{fig:prompt_example}{{2}{7}{Textual representation of the top grid in the ``interaction phase'' of \Cref {fig:pipeline_overview}}{figure.caption.37}{}}
\newlabel{fig:prompt_example@cref}{{[figure][2][]2}{[1][7][]7}{}{}{}}
\csxdef {autonum@sec:text-interfaceReferenced}{}
\@writefile{toc}{\contentsline {subsection}{\numberline {5.2}Results}{7}{subsection.46}\protected@file@percent }
\newlabel{sec:results}{{5.2}{7}{}{subsection.46}{}}
\newlabel{sec:results@cref}{{[subsection][2][5]5.2}{[1][7][]7}{}{}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {5.2.1}Overall Performance}{7}{subsubsection.47}\protected@file@percent }
\csxdef {autonum@fig:score_by_task_typeReferenced}{}
\csxdef {autonum@tab:avg_scoresReferenced}{}
\csxdef {autonum@fig:score_by_env_violinReferenced}{}
\csxdef {autonum@fig:stochastic_vs_detReferenced}{}
\csxdef {autonum@fig:perf-costReferenced}{}
\@writefile{lof}{\contentsline {figure}{\numberline {4}{\ignorespaces Score vs. cost per problem across environments.}}{7}{figure.caption.48}\protected@file@percent }
\newlabel{fig:perf-cost}{{4}{7}{Score vs. cost per problem across environments}{figure.caption.48}{}}
\newlabel{fig:perf-cost@cref}{{[figure][4][]4}{[1][7][]7}{}{}{}}
\csxdef {autonum@sec:cost-performanceReferenced}{}
\csxdef {autonum@sec:detailed-performanceReferenced}{}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {5.2.2}Exploration Patterns}{7}{subsubsection.49}\protected@file@percent }
\BKM@entry{id=14,dest={73756273756273656374696F6E2E3532},srcline={1318}}{5C3337365C3337375C303030575C3030306F5C303030725C3030306C5C303030645C3030302D5C3030304D5C3030306F5C303030645C303030655C3030306C5C3030305C3034305C3030304C5C303030655C303030615C303030725C3030306E5C303030695C3030306E5C30303067}
\BKM@entry{id=15,dest={73756273656374696F6E2E3533},srcline={1345}}{5C3337365C3337375C303030445C303030695C303030735C303030635C303030755C303030735C303030735C303030695C3030306F5C3030306E}
\newlabel{fig:reset_by_env_violin}{{6a}{8}{Resets}{figure.caption.50}{}}
\newlabel{fig:reset_by_env_violin@cref}{{[subfigure][1][6]6a}{[1][7][]8}{}{}{}}
\newlabel{sub@fig:reset_by_env_violin}{{a}{8}{Resets}{figure.caption.50}{}}
\newlabel{sub@fig:reset_by_env_violin@cref}{{[subfigure][1][6]6a}{[1][7][]8}{}{}{}}
\newlabel{fig:auc_by_env_violin}{{6b}{8}{AUC}{figure.caption.50}{}}
\newlabel{fig:auc_by_env_violin@cref}{{[subfigure][2][6]6b}{[1][7][]8}{}{}{}}
\newlabel{sub@fig:auc_by_env_violin}{{b}{8}{AUC}{figure.caption.50}{}}
\newlabel{sub@fig:auc_by_env_violin@cref}{{[subfigure][2][6]6b}{[1][7][]8}{}{}{}}
\newlabel{fig:final_perplexity_by_env_violin}{{6c}{8}{Final perplexity}{figure.caption.50}{}}
\newlabel{fig:final_perplexity_by_env_violin@cref}{{[subfigure][3][6]6c}{[1][7][]8}{}{}{}}
\newlabel{sub@fig:final_perplexity_by_env_violin}{{c}{8}{Final perplexity}{figure.caption.50}{}}
\newlabel{sub@fig:final_perplexity_by_env_violin@cref}{{[subfigure][3][6]6c}{[1][7][]8}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {6}{\ignorespaces Environment-specific performance and behavioral metrics. (a) Reset frequency distributions, (b) Area Under the Curve (AUC) for normalized perplexities, and (c) Final perplexity values.}}{8}{figure.caption.50}\protected@file@percent }
\newlabel{fig:perf_env_grid}{{6}{8}{Environment-specific performance and behavioral metrics. (a) Reset frequency distributions, (b) Area Under the Curve (AUC) for normalized perplexities, and (c) Final perplexity values}{figure.caption.50}{}}
\newlabel{fig:perf_env_grid@cref}{{[figure][6][]6}{[1][7][]8}{}{}{}}
\csxdef {autonum@fig:actions_distributionReferenced}{}
\@writefile{lof}{\contentsline {figure}{\numberline {5}{\ignorespaces Action type distribution per agent averaged over AutumnBench problems.}}{8}{figure.caption.51}\protected@file@percent }
\newlabel{fig:actions_distribution}{{5}{8}{Action type distribution per agent averaged over AutumnBench problems}{figure.caption.51}{}}
\newlabel{fig:actions_distribution@cref}{{[figure][5][]5}{[1][7][]8}{}{}{}}
\csxdef {autonum@fig:reset_by_env_violinReferenced}{}
\csxdef {autonum@tab:avg_actionsReferenced}{}
\csxdef {autonum@sec:lcs-analysisReferenced}{}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {5.2.3}World-Model Learning}{8}{subsubsection.52}\protected@file@percent }
\csxdef {autonum@def:norm_perplexityReferenced}{}
\csxdef {autonum@def:aucReferenced}{}
\csxdef {autonum@fig:auc_by_env_violinReferenced}{}
\csxdef {autonum@fig:final_perplexity_by_env_violinReferenced}{}
\csxdef {autonum@fig:perf_env_gridReferenced}{}
\@writefile{toc}{\contentsline {subsection}{\numberline {5.3}Discussion}{8}{subsection.53}\protected@file@percent }
\newlabel{sec:discussion}{{5.3}{8}{}{subsection.53}{}}
\newlabel{sec:discussion@cref}{{[subsection][3][5]5.3}{[1][8][]8}{}{}{}}
\@writefile{toc}{\contentsline {paragraph}{Experimental design.}{8}{subsection.53}\protected@file@percent }
\csxdef {autonum@lst:example_scratchpadReferenced}{}
\BKM@entry{id=16,dest={73656374696F6E2E3534},srcline={1380}}{5C3337365C3337375C303030435C3030306F5C3030306E5C303030635C3030306C5C303030755C303030735C303030695C3030306F5C3030306E}
\citation{warrier2026autumnbench}
\bibstyle{icml2026}
\bibdata{main}
\bibcite{causalworld}{{1}{2021}{{Ahmed et~al.}}{{Ahmed, Tr{\"a}uble, Goyal, Neitz, W{\"u}thrich, Bengio, Sch{\"o}lkopf, and Bauer}}}
\csxdef {autonum@fig:actions_distributionReferenced}{}
\@writefile{toc}{\contentsline {paragraph}{Belief updating.}{9}{subsection.53}\protected@file@percent }
\csxdef {autonum@lst:example_scratchpadReferenced}{}
\@writefile{toc}{\contentsline {section}{\numberline {6}Conclusion}{9}{section.54}\protected@file@percent }
\newlabel{sec:conclusion}{{6}{9}{}{section.54}{}}
\newlabel{sec:conclusion@cref}{{[section][6][]6}{[1][9][]9}{}{}{}}
\csxdef {autonum@sec:prompt-robustnessReferenced}{}
\bibcite{autumnbench_dataset}{{2}{2025}{{Anonymous}}{{}}}
\bibcite{phyre}{{3}{2019}{{Bakhtin et~al.}}{{Bakhtin, Johnson, Gkioxari, Girshick, Riedmiller, and Lerer}}}
\bibcite{pgm}{{4}{2018}{{Barrett et~al.}}{{Barrett, Hill, Santoro, Morcos, and Lillicrap}}}
\bibcite{bellemare2013arcade}{{5}{2013}{{Bellemare et~al.}}{{Bellemare, Naddaf, Veness, and Bowling}}}
\bibcite{bramley2018intuitive}{{6}{2018}{{Bramley et~al.}}{{Bramley, Gerstenberg, Tenenbaum, and Gureckis}}}
\bibcite{brockman2016openai}{{7}{2016}{{Brockman et~al.}}{{Brockman, Cheung, Pettersson, Schneider, Schulman, Tang, and Zaremba}}}
\bibcite{arc_paper}{{8}{2019}{{Chollet}}{{}}}
\bibcite{procgen}{{9}{2020}{{Cobbe et~al.}}{{Cobbe, Hesse, Hilton, and Schulman}}}
\bibcite{coenen2015strategies}{{10}{2015}{{Coenen et~al.}}{{Coenen, Rehder, and Gureckis}}}
\bibcite{autumnsynth}{{11}{2023}{{Das et~al.}}{{Das, Tenenbaum, Solar-Lezama, and Tavares}}}
\bibcite{bongard}{{12}{2018}{{Depeweg et~al.}}{{Depeweg, Rothkopf, and J\"{a}kel}}}
\bibcite{Douglas2023}{{13}{2023}{{Douglas et~al.}}{{Douglas, Ewell, and Brauer}}}
\bibcite{bairrobotpushing}{{14}{2017}{{Ebert et~al.}}{{Ebert, Finn, Lee, and Levine}}}
\bibcite{puzzles}{{15}{2024}{{Estermann et~al.}}{{Estermann, Lanzend\"{o}rfer, Niedermayr, and Wattenhofer}}}
\bibcite{girdhar2020cater}{{16}{2020}{{Girdhar \& Ramanan}}{{Girdhar and Ramanan}}}
\bibcite{dreamerv3}{{17}{2025}{{Hafner et~al.}}{{Hafner, Pasukonis, Ba, and Lillicrap}}}
\bibcite{vbench}{{18}{2024}{{Huang et~al.}}{{Huang, He, Yu, Zhang, Si, Jiang, Zhang, Wu, Jin, Chanpaisit, Wang, Chen, Wang, Lin, Qiao, and Liu}}}
\bibcite{discoveryworld}{{19}{2024}{{Jansen et~al.}}{{Jansen, C\^{o}t\'{e}, Khot, Bransom, Dalvi~Mishra, Majumder, Tafjord, and Clark}}}
\bibcite{jimenez2024swebench}{{20}{2024}{{Jimenez et~al.}}{{Jimenez, Yang, Wettig, Yao, Pei, Press, and Narasimhan}}}
\bibcite{svib}{{21}{2023}{{Kim et~al.}}{{Kim, Singh, Park, Gulcehre, and Ahn}}}
\bibcite{nethack}{{22}{2023}{{K{\"u}ttler et~al.}}{{K{\"u}ttler, Nardelli, Miller, Raileanu, Grefenstette, Timsin, et~al.}}}
\bibcite{laskin2021urlbunsupervisedreinforcementlearning}{{23}{2021}{{Laskin et~al.}}{{Laskin, Yarats, Liu, Lee, Zhan, Lu, Cang, Pinto, and Abbeel}}}
\bibcite{laskin2023ad}{{24}{2023}{{Laskin et~al.}}{{Laskin, Wang, Oh, Parisotto, Spencer, Steiber, Strouse, Hansen, Filos, Brooks, Gazeau, Sahni, Singh, and Mnih}}}
\bibcite{LeCun2022APT}{{25}{2022}{{LeCun}}{{}}}
\bibcite{li24simpler}{{26}{2024}{{Li et~al.}}{{Li, Hsu, Gu, Pertsch, Mees, Walke, Fu, Lunawat, Sieh, Kirmani, Levine, Wu, Finn, Su, Vuong, and Xiao}}}
\bibcite{terminalbench}{{27}{2026}{{Merrill et~al.}}{{Merrill, Shaw, Carlini, Li, Raj, Bercovich, Shi, Shin, Walshe, Buchanan, Shen, Ye, Lin, Poulos, Wang, Jitsev, Nezhurina, Lu, Mastromichalakis, Xu, Chen, Liu, Zhang, Chen, Kashyap, Uslu, Li, Wu, Yan, Bian, Sharma, Sun, Dillmann, Anand, Lanpouthakoun, Koopah, Hu, Guha, Dreiman, Zhu, Krauth, Zhong, Muennighoff, Amanfu, Tan, Pimpalgaonkar, Aggarwal, Lin, Lan, Zhao, Liang, Wang, Wang, Zhou, Heineman, Liu, Trivedi, Yang, Lin, Shetty, Yang, Omi, Raoof, Li, Zhuo, Lin, Dai, Wang, Chai, Zhou, Wahdany, She, Hu, Dong, Zhu, Cui, Saiyed, Kolbeinsson, Rytting, Marten, Wang, Dimakis, Konwinski, and Schmidt}}}
\bibcite{Muszyski2023}{{28}{2023}{{Muszy\'{n}ski}}{{}}}
\bibcite{prolific}{{29}{2025}{{Prolific}}{{}}}
\bibcite{reid2022softwareengineeringuserstudy}{{30}{2022}{{Reid et~al.}}{{Reid, Wagner, d'Amorim, and Treude}}}
\bibcite{rein2024gpqa}{{31}{2024}{{Rein et~al.}}{{Rein, Hou, Stickland, Petty, Pang, Dirani, Michael, and Bowman}}}
\bibcite{minihack}{{32}{2021}{{Samvelyan et~al.}}{{Samvelyan, Kirk, Kurin, Parker-Holder, Jiang, Hambro, Petroni, Kuttler, Grefenstette, and Rockt{\"a}schel}}}
\bibcite{movingmnist}{{33}{2015}{{Srivastava et~al.}}{{Srivastava, Mansimov, and Salakhutdinov}}}
\bibcite{dmcsuite}{{34}{2020}{{Tunyasuvunakool et~al.}}{{Tunyasuvunakool, Muldal, Doron, Liu, Bohez, Merel, Erez, Lillicrap, Heess, and Tassa}}}
\bibcite{wang2026context}{{35}{2026}{{Wang et~al.}}{{Wang, Chen, Zhong, Zheng, Shao, Yu, Liu, Wang, Ding, Cao, and Kang}}}
\bibcite{alchemy}{{36}{2021}{{Wang et~al.}}{{Wang, King, Porcel, Kurth-Nelson, Zhu, Deck, Choy, Cassin, Reynolds, Song, Buttimore, Reichert, Rabinowitz, Matthey, Hassabis, Lerchner, and Botvinick}}}
\bibcite{warrier2026autumnbench}{{37}{2026}{{Warrier et~al.}}{{Warrier, Nguyen, Naim, Jain, Liang, Schroeder, Yang, Tenenbaum, Vollmer, Ellis, and Tavares}}}
\bibcite{Weisberg2013}{{38}{2013}{{Weisberg \& Gopnik}}{{Weisberg and Gopnik}}}
\bibcite{nim}{{39}{2025}{{Wikipedia}}{{}}}
\bibcite{kexin2021clevrer}{{40}{2020}{{Yi et~al.}}{{Yi, Gan, Li, Kohli, Wu, Torralba, and Tenenbaum}}}
\bibcite{lance2025assessing}{{41}{2025}{{Ying et~al.}}{{Ying, Collins, Sharma, Colas, Zhao, Weller, Tavares, Isola, Gershman, Andreas, Griffiths, Chollet, Allen, and Tenenbaum}}}
\bibcite{raven}{{42}{2019}{{Zhang et~al.}}{{Zhang, Gao, Jia, Zhu, and Zhu}}}
\bibcite{acre}{{43}{2020}{{Zhang et~al.}}{{Zhang, Jia, Yang, and Zhu}}}
\BKM@entry{id=17,dest={617070656E6469782E3630},srcline={1}}{5C3337365C3337375C303030545C303030685C303030655C3030305C3034305C303030415C303030755C303030745C303030755C3030306D5C3030306E5C3030305C3034305C3030304C5C303030615C3030306E5C303030675C303030755C303030615C303030675C30303065}
\citation{autumnsynth}
\@writefile{toc}{\contentsline {section}{\numberline {A}The Autumn Language}{13}{appendix.60}\protected@file@percent }
\newlabel{sec:autumn}{{A}{13}{Impact Statement}{appendix.60}{}}
\newlabel{sec:autumn@cref}{{[appendix][1][]A}{[1][13][]13}{}{}{}}
\@writefile{toc}{\contentsline {paragraph}{Example Autumn Environment.}{13}{Item.63}\protected@file@percent }
\csxdef {autonum@lst:autumn_light_bar_exampleReferenced}{}
\csxdef {autonum@fig:treasure_environmentReferenced}{}
\savepointas{setupstart}{pgfid86}{0pt}{0pt}
\savepicturepage{pgfid86}{13}
\pgfsyspdfmark {pgfid86}{3646961}{20303547}
\savepointas{setupend}{pgfid87}{0pt}{0pt}
\savepicturepage{pgfid87}{13}
\pgfsyspdfmark {pgfid87}{12612263}{20303547}
\savepointas{objectstart}{pgfid88}{0pt}{0pt}
\savepicturepage{pgfid88}{13}
\pgfsyspdfmark {pgfid88}{3646961}{19386043}
\savepointas{objectend}{pgfid89}{0pt}{0pt}
\savepicturepage{pgfid89}{13}
\pgfsyspdfmark {pgfid89}{19690133}{17551035}
\savepointas{oninstancestart}{pgfid90}{0pt}{0pt}
\savepicturepage{pgfid90}{13}
\pgfsyspdfmark {pgfid90}{3646961}{16633531}
\savepointas{oninstanceend}{pgfid91}{0pt}{0pt}
\savepicturepage{pgfid91}{13}
\pgfsyspdfmark {pgfid91}{23229068}{13422267}
\savepointas{onstart}{pgfid92}{0pt}{0pt}
\savepicturepage{pgfid92}{13}
\pgfsyspdfmark {pgfid92}{3646961}{12504763}
\savepointas{onend}{pgfid93}{0pt}{0pt}
\savepicturepage{pgfid93}{13}
\pgfsyspdfmark {pgfid93}{20633849}{9752251}
\savepicturepage{pgfid94}{13}
\pgfsyspdfmark {pgfid94}{3646961}{8434976}
\@writefile{lol}{\contentsline {listing}{\numberline {A.1}{\ignorespaces A treasure-hunting environment example in Autumn. Interactive demo available at \href  {https://autumn.basis.ai/build-mode?code=KHByb2dyYW0KICAgKD0gR1JJRF9TSVpFIDUpCiAgIChvYmplY3QgUHJveGltaXR5ICg6IGRpc3QgTnVtYmVyKQogICAgIChtYXAgKC0tPiAoaSkgKENlbGwgaSAwIChpZiAoPD0gaSBkaXN0KSB0aGVuICJibHVlIiBlbHNlICJibGFjayIpKSkKICAgICAgICAgIChyYW5nZSAwIEdSSURfU0laRSkpKQogICAob2JqZWN0IFRyZWFzdXJlICg6IHJldmVhbGVkIEJvb2wpIChDZWxsIDAgMCAoaWYgcmV2ZWFsZWQgdGhlbiAiZ29sZCIgZWxzZSAiYmxhY2siKSkpCiAgIChvYmplY3QgQWdlbnQgKENlbGwgMCAwICJncmV5IikpCgogICAoOiB0cmVhc3VyZXMgKExpc3QgVHJlYXN1cmUpKQogICAoPSB0cmVhc3VyZXMgKGluaXRuZXh0IChsZXQKICAgICg9IHBvczEgKHVuaWZvcm1DaG9pY2UgKHJlY3QgKFBvc2l0aW9uIDAgMSkgKFBvc2l0aW9uIEdSSURfU0laRSBHUklEX1NJWkUpKSkpCiAgICAoPSBwb3MyICh1bmlmb3JtQ2hvaWNlIChmaWx0ZXIgKC0tPiBwICghICgmICg9PSAoLi4gcCB4KSAoLi4gcG9zMSB4KSkgKD09ICguLiBwIHkpICguLiBwb3MxIHkpKSkpKSAocmVjdCAoUG9zaXRpb24gMCAxKSAoUG9zaXRpb24gR1JJRF9TSVpFIEdSSURfU0laRSkpKSkpCiAgICAoPSBwb3MzICh1bmlmb3JtQ2hvaWNlIChmaWx0ZXIgKC0tPiBwICghICgmIChpbiAoLi4gcCB4KSAobGlzdCAoLi4gcG9zMSB4KSAoLi4gcG9zMiB4KSkpIChpbiAoLi4gcCB5KSAobGlzdCAoLi4gcG9zMSB5KSAoLi4gcG9zMiB5KSkpKSkpIChyZWN0IChQb3NpdGlvbiAwIDEpIChQb3NpdGlvbiBHUklEX1NJWkUgR1JJRF9TSVpFKSkpKSkKICAgIChwcmludCBwb3MzKQogICAgKGxpc3QgKFRyZWFzdXJlIHRydWUgcG9zMSkgKFRyZWFzdXJlIHRydWUgcG9zMikgKFRyZWFzdXJlIGZhbHNlIHBvczMpKQogICApIChwcmV2IHRyZWFzdXJlcykpKQoKICAgKDogYWdlbnQgQWdlbnQpCiAgICg9IGFnZW50IChpbml0bmV4dCAoQWdlbnQgKFBvc2l0aW9uIDAgMSkpIChwcmV2IGFnZW50KSkpCgogICA7IGNhbGN1bGF0ZSB0aGUgZGlzdGFuY2UgdG8gdGhlIGNsb3Nlc3QgdHJlYXN1cmUKICAgKD0gdGRpc3QgKGZuICh0cmVhc3VyZXMpCiAgICAoc3FkaXN0ICguLiBhZ2VudCBvcmlnaW4pICguLiAoY2xvc2VzdCBhZ2VudCB0cmVhc3VyZXMpIG9yaWdpbikpCiAgICkpCgogICAoOiBwcm94aW1pdHkgUHJveGltaXR5KQogICAoPSBwcm94aW1pdHkgKGluaXRuZXh0IChQcm94aW1pdHkgMiAoUG9zaXRpb24gMCAwKSkKICAgICAgKHVwZGF0ZU9iaiBwcm94aW1pdHkgImRpc3QiICgrICh0ZGlzdCB0cmVhc3VyZXMpICgtICh1bmlmb3JtQ2hvaWNlIChyYW5nZSAwIDMpKSAxKSkpKSkKCiAgIChvbiB1cCAoPSBhZ2VudCAobW92ZVVwIGFnZW50KSkpCiAgIChvbiBkb3duICg9IGFnZW50IChtb3ZlRG93biBhZ2VudCkpKQogICAob24gbGVmdCAoPSBhZ2VudCAobW92ZUxlZnQgYWdlbnQpKSkKICAgKG9uIHJpZ2h0ICg9IGFnZW50IChtb3ZlUmlnaHQgYWdlbnQpKSkKICAgKG9uIChjbGlja2VkIHRyZWFzdXJlcykgKD0gdHJlYXN1cmVzICh1cGRhdGVPYmogdHJlYXN1cmVzICgtLT4gb2JqICh1cGRhdGVPYmogb2JqICJyZXZlYWxlZCIgdHJ1ZSkpICgtLT4gb2JqIChjbGlja2VkIG9iaikpKSkpCiAgKQo=}{\texttt  {autumn.basis.ai}.}}}{13}{listing.89}\protected@file@percent }
\newlabel{lst:autumn_light_bar_example}{{A.1}{13}{A treasure-hunting environment example in Autumn.\onlyinarxiv { Interactive demo available at \href {\detokenize {https://autumn.basis.ai/build-mode?code=KHByb2dyYW0KICAgKD0gR1JJRF9TSVpFIDUpCiAgIChvYmplY3QgUHJveGltaXR5ICg6IGRpc3QgTnVtYmVyKQogICAgIChtYXAgKC0tPiAoaSkgKENlbGwgaSAwIChpZiAoPD0gaSBkaXN0KSB0aGVuICJibHVlIiBlbHNlICJibGFjayIpKSkKICAgICAgICAgIChyYW5nZSAwIEdSSURfU0laRSkpKQogICAob2JqZWN0IFRyZWFzdXJlICg6IHJldmVhbGVkIEJvb2wpIChDZWxsIDAgMCAoaWYgcmV2ZWFsZWQgdGhlbiAiZ29sZCIgZWxzZSAiYmxhY2siKSkpCiAgIChvYmplY3QgQWdlbnQgKENlbGwgMCAwICJncmV5IikpCgogICAoOiB0cmVhc3VyZXMgKExpc3QgVHJlYXN1cmUpKQogICAoPSB0cmVhc3VyZXMgKGluaXRuZXh0IChsZXQKICAgICg9IHBvczEgKHVuaWZvcm1DaG9pY2UgKHJlY3QgKFBvc2l0aW9uIDAgMSkgKFBvc2l0aW9uIEdSSURfU0laRSBHUklEX1NJWkUpKSkpCiAgICAoPSBwb3MyICh1bmlmb3JtQ2hvaWNlIChmaWx0ZXIgKC0tPiBwICghICgmICg9PSAoLi4gcCB4KSAoLi4gcG9zMSB4KSkgKD09ICguLiBwIHkpICguLiBwb3MxIHkpKSkpKSAocmVjdCAoUG9zaXRpb24gMCAxKSAoUG9zaXRpb24gR1JJRF9TSVpFIEdSSURfU0laRSkpKSkpCiAgICAoPSBwb3MzICh1bmlmb3JtQ2hvaWNlIChmaWx0ZXIgKC0tPiBwICghICgmIChpbiAoLi4gcCB4KSAobGlzdCAoLi4gcG9zMSB4KSAoLi4gcG9zMiB4KSkpIChpbiAoLi4gcCB5KSAobGlzdCAoLi4gcG9zMSB5KSAoLi4gcG9zMiB5KSkpKSkpIChyZWN0IChQb3NpdGlvbiAwIDEpIChQb3NpdGlvbiBHUklEX1NJWkUgR1JJRF9TSVpFKSkpKSkKICAgIChwcmludCBwb3MzKQogICAgKGxpc3QgKFRyZWFzdXJlIHRydWUgcG9zMSkgKFRyZWFzdXJlIHRydWUgcG9zMikgKFRyZWFzdXJlIGZhbHNlIHBvczMpKQogICApIChwcmV2IHRyZWFzdXJlcykpKQoKICAgKDogYWdlbnQgQWdlbnQpCiAgICg9IGFnZW50IChpbml0bmV4dCAoQWdlbnQgKFBvc2l0aW9uIDAgMSkpIChwcmV2IGFnZW50KSkpCgogICA7IGNhbGN1bGF0ZSB0aGUgZGlzdGFuY2UgdG8gdGhlIGNsb3Nlc3QgdHJlYXN1cmUKICAgKD0gdGRpc3QgKGZuICh0cmVhc3VyZXMpCiAgICAoc3FkaXN0ICguLiBhZ2VudCBvcmlnaW4pICguLiAoY2xvc2VzdCBhZ2VudCB0cmVhc3VyZXMpIG9yaWdpbikpCiAgICkpCgogICAoOiBwcm94aW1pdHkgUHJveGltaXR5KQogICAoPSBwcm94aW1pdHkgKGluaXRuZXh0IChQcm94aW1pdHkgMiAoUG9zaXRpb24gMCAwKSkKICAgICAgKHVwZGF0ZU9iaiBwcm94aW1pdHkgImRpc3QiICgrICh0ZGlzdCB0cmVhc3VyZXMpICgtICh1bmlmb3JtQ2hvaWNlIChyYW5nZSAwIDMpKSAxKSkpKSkKCiAgIChvbiB1cCAoPSBhZ2VudCAobW92ZVVwIGFnZW50KSkpCiAgIChvbiBkb3duICg9IGFnZW50IChtb3ZlRG93biBhZ2VudCkpKQogICAob24gbGVmdCAoPSBhZ2VudCAobW92ZUxlZnQgYWdlbnQpKSkKICAgKG9uIHJpZ2h0ICg9IGFnZW50IChtb3ZlUmlnaHQgYWdlbnQpKSkKICAgKG9uIChjbGlja2VkIHRyZWFzdXJlcykgKD0gdHJlYXN1cmVzICh1cGRhdGVPYmogdHJlYXN1cmVzICgtLT4gb2JqICh1cGRhdGVPYmogb2JqICJyZXZlYWxlZCIgdHJ1ZSkpICgtLT4gb2JqIChjbGlja2VkIG9iaikpKSkpCiAgKQo=}}{\texttt {autumn.basis.ai}.}}}{listing.89}{}}
\newlabel{lst:autumn_light_bar_example@cref}{{[listing][1][1]A.1}{[1][13][]13}{}{}{}}
\BKM@entry{id=18,dest={617070656E6469782E3931},srcline={121}}{5C3337365C3337375C303030415C303030755C303030745C303030755C3030306D5C3030306E5C303030425C303030655C3030306E5C303030635C303030685C3030305C3034305C303030455C3030306E5C303030765C303030695C303030725C3030306F5C3030306E5C3030306D5C303030655C3030306E5C303030745C3030305C3034305C303030445C303030655C303030745C303030615C303030695C3030306C5C30303073}
\@writefile{lof}{\contentsline {figure}{\numberline {A.1}{\ignorespaces Renderings of a partial trajectory of the Autumn environment example from \autonum@processReference {autonum@referenceCrefOld}{forcsvlist}{lst:autumn_light_bar_example}, following the sequence of actions down, down, down and click(1, 4).}}{14}{figure.caption.90}\protected@file@percent }
\csxdef {autonum@lst:autumn_light_bar_exampleReferenced}{}
\newlabel{fig:treasure_environment}{{A.1}{14}{Renderings of a partial trajectory of the Autumn environment example from \Cref {lst:autumn_light_bar_example}, following the sequence of actions down, down, down and click(1, 4)}{figure.caption.90}{}}
\newlabel{fig:treasure_environment@cref}{{[figure][1][1]A.1}{[1][13][]14}{}{}{}}
\@writefile{toc}{\contentsline {section}{\numberline {B}AutumnBench Environment Details}{14}{appendix.91}\protected@file@percent }
\newlabel{sec:env_details}{{B}{14}{Impact Statement}{appendix.91}{}}
\newlabel{sec:env_details@cref}{{[appendix][2][]B}{[1][14][]14}{}{}{}}
\csxdef {autonum@tab:env_categoriesReferenced}{}
\csxdef {autonum@tab:program_statsReferenced}{}
\@writefile{lot}{\contentsline {table}{\numberline {B.1}{\ignorespaces Category tags for each AutumnBench environment. Labels are non-exclusive.}}{15}{table.caption.92}\protected@file@percent }
\newlabel{tab:env_categories}{{B.1}{15}{Category tags for each AutumnBench environment. Labels are non-exclusive}{table.caption.92}{}}
\newlabel{tab:env_categories@cref}{{[table][1][2]B.1}{[1][14][]15}{}{}{}}
\@writefile{lot}{\contentsline {table}{\numberline {B.2}{\ignorespaces Program statistics for all AutumnBench environments. Columns: number of object types (\#Obj), number of latent variables (\#Lat., i.e.\ Autumn program fields not rendered on the grid), program length in lines of code (Len.), number of event handlers (\#On), number of colors (\#Col.), and grid size. \textbf  {Left:} deterministic environments. \textbf  {Right:} stochastic environments.}}{15}{table.caption.93}\protected@file@percent }
\newlabel{tab:program_stats}{{B.2}{15}{Program statistics for all AutumnBench environments. Columns: number of object types (\#Obj), number of latent variables (\#Lat., i.e.\ Autumn program fields not rendered on the grid), program length in lines of code (Len.), number of event handlers (\#On), number of colors (\#Col.), and grid size. \textbf {Left:} deterministic environments. \textbf {Right:} stochastic environments}{table.caption.93}{}}
\newlabel{tab:program_stats@cref}{{[table][2][2]B.2}{[1][14][]15}{}{}{}}
\BKM@entry{id=19,dest={617070656E6469782E3934},srcline={252}}{5C3337365C3337375C303030415C303030755C303030745C303030755C3030306D5C3030306E5C303030425C303030655C3030306E5C303030635C303030685C3030305C3034305C303030435C303030685C303030615C3030306C5C3030306C5C303030655C3030306E5C303030675C303030655C3030305C3034305C303030465C3030306F5C303030725C3030306D5C303030755C3030306C5C303030615C303030745C303030695C3030306F5C3030306E}
\BKM@entry{id=20,dest={73756273656374696F6E2E3935},srcline={257}}{5C3337365C3337375C3030304D5C303030615C303030735C3030306B5C303030655C303030645C3030305C3034305C303030465C303030725C303030615C3030306D5C303030655C3030305C3034305C303030505C303030725C303030655C303030645C303030695C303030635C303030745C303030695C3030306F5C3030306E}
\BKM@entry{id=21,dest={73756273656374696F6E2E3936},srcline={268}}{5C3337365C3337375C303030435C303030685C303030615C3030306E5C303030675C303030655C3030305C3034305C303030445C303030655C303030745C303030655C303030635C303030745C303030695C3030306F5C3030306E}
\BKM@entry{id=22,dest={73756273656374696F6E2E3939},srcline={290}}{5C3337365C3337375C303030505C3030306C5C303030615C3030306E5C3030306E5C303030695C3030306E5C30303067}
\BKM@entry{id=23,dest={617070656E6469782E313030},srcline={296}}{5C3337365C3337375C303030495C3030306D5C303030705C3030306C5C303030655C3030306D5C303030655C3030306E5C303030745C303030615C303030745C303030695C3030306F5C3030306E5C3030305C3034305C303030445C303030655C303030745C303030615C303030695C3030306C5C30303073}
\BKM@entry{id=24,dest={73756273656374696F6E2E313031},srcline={301}}{5C3337365C3337375C3030304E5C3030306F5C303030725C3030306D5C303030615C3030306C5C303030695C3030307A5C303030655C303030645C3030305C3034305C303030505C303030655C303030725C303030705C3030306C5C303030655C303030785C303030695C303030745C30303079}
\@writefile{toc}{\contentsline {section}{\numberline {C}AutumnBench Challenge Formulation}{16}{appendix.94}\protected@file@percent }
\newlabel{sec:challenge-formulation}{{C}{16}{Impact Statement}{appendix.94}{}}
\newlabel{sec:challenge-formulation@cref}{{[appendix][3][]C}{[1][16][]16}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {C.1}Masked Frame Prediction}{16}{subsection.95}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {C.2}Change Detection}{16}{subsection.96}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {C.3}Planning}{16}{subsection.99}\protected@file@percent }
\@writefile{toc}{\contentsline {section}{\numberline {D}Implementation Details}{16}{appendix.100}\protected@file@percent }
\newlabel{sec:impl_details}{{D}{16}{Impact Statement}{appendix.100}{}}
\newlabel{sec:impl_details@cref}{{[appendix][4][]D}{[1][16][]16}{}{}{}}
\BKM@entry{id=25,dest={73756273656374696F6E2E313034},srcline={324}}{5C3337365C3337375C303030545C303030615C303030735C3030306B5C3030305C3034305C303030495C3030306E5C303030745C303030655C303030725C303030665C303030615C303030635C303030655C3030305C3034305C303030495C3030306D5C303030705C3030306C5C303030655C3030306D5C303030655C3030306E5C303030745C303030615C303030745C303030695C3030306F5C3030306E}
\BKM@entry{id=26,dest={73756273756273656374696F6E2E313035},srcline={328}}{5C3337365C3337375C303030475C303030725C303030615C303030705C303030685C303030695C303030635C303030615C3030306C5C3030305C3034305C303030555C303030735C303030655C303030725C3030305C3034305C303030495C3030306E5C303030745C303030655C303030725C303030665C303030615C303030635C30303065}
\@writefile{toc}{\contentsline {subsection}{\numberline {D.1}Normalized Perplexity}{17}{subsection.101}\protected@file@percent }
\newlabel{def:norm_perplexity}{{D.1}{17}{Normalized Perplexity}{definition.1.D.1}{}}
\newlabel{def:norm_perplexity@cref}{{[definition][1][4]D.1}{[1][16][]17}{}{}{}}
\newlabel{def:auc}{{D.2}{17}{Area Under the Curve (AUC) of Normalized Perplexity}{definition.1.D.2}{}}
\newlabel{def:auc@cref}{{[definition][2][4]D.2}{[1][17][]17}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {D.2}Task Interface Implementation}{17}{subsection.104}\protected@file@percent }
\@writefile{toc}{\contentsline {subsubsection}{\numberline {D.2.1}Graphical User Interface}{17}{subsubsection.105}\protected@file@percent }
\newlabel{sec:task-gui}{{D.2.1}{17}{Final Normalized Perplexity}{subsubsection.105}{}}
\newlabel{sec:task-gui@cref}{{[subsubsection][1][4,2]D.2.1}{[1][17][]17}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {D.1}{\ignorespaces Example of masked frame prediction task on the AutumnBench GUI showing the slider, action viewer, six choice options, and a \texttt  {Submit} button.}}{17}{figure.caption.106}\protected@file@percent }
\newlabel{fig:mfp-grid}{{D.1}{17}{Example of masked frame prediction task on the AutumnBench GUI showing the slider, action viewer, six choice options, and a \texttt {Submit} button}{figure.caption.106}{}}
\newlabel{fig:mfp-grid@cref}{{[figure][1][4]D.1}{[1][17][]17}{}{}{}}
\csxdef {autonum@fig:mfp-gridReferenced}{}
\@writefile{lof}{\contentsline {figure}{\numberline {D.7}{\ignorespaces Example of planning task on the AutumnBench GUI that shows a target region by masking out cells that are not in the target.}}{17}{figure.caption.107}\protected@file@percent }
\newlabel{fig:planning-grid}{{D.7}{17}{Example of planning task on the AutumnBench GUI that shows a target region by masking out cells that are not in the target}{figure.caption.107}{}}
\newlabel{fig:planning-grid@cref}{{[figure][7][4]D.7}{[1][17][]17}{}{}{}}
\csxdef {autonum@fig:planning-gridReferenced}{}
\@writefile{lof}{\contentsline {figure}{\numberline {D.8}{\ignorespaces Change detection on the AutumnBench GUI. (a) Initial change detection phase with \texttt  {Reset} and \texttt  {Found change} buttons. (b) Frame selection phase with the action viewer, slider, and \texttt  {Submit} button.}}{18}{figure.caption.108}\protected@file@percent }
\newlabel{fig:change-detection-grid}{{D.8}{18}{Change detection on the AutumnBench GUI. (a) Initial change detection phase with \texttt {Reset} and \texttt {Found change} buttons. (b) Frame selection phase with the action viewer, slider, and \texttt {Submit} button}{figure.caption.108}{}}
\newlabel{fig:change-detection-grid@cref}{{[figure][8][4]D.8}{[1][17][]18}{}{}{}}
\csxdef {autonum@fig:change-detection-gridReferenced}{}
\BKM@entry{id=27,dest={73756273756273656374696F6E2E313039},srcline={382}}{5C3337365C3337375C303030545C303030655C303030785C303030745C3030302D5C303030425C303030615C303030735C303030655C303030645C3030305C3034305C303030495C3030306E5C303030745C303030655C303030725C303030665C303030615C303030635C30303065}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {D.2.2}Text-Based Interface}{19}{subsubsection.109}\protected@file@percent }
\newlabel{sec:text-interface}{{D.2.2}{19}{Final Normalized Perplexity}{subsubsection.109}{}}
\newlabel{sec:text-interface@cref}{{[subsubsection][2][4,2]D.2.2}{[1][19][]19}{}{}{}}
\csxdef {autonum@lst:sys-promptReferenced}{}
\csxdef {autonum@lst:mfp-promptReferenced}{}
\csxdef {autonum@lst:planning-promptReferenced}{}
\csxdef {autonum@lst:change-detection-promptReferenced}{}
\@writefile{lol}{\contentsline {listing}{\numberline {D.1}{\ignorespaces System prompt for all reasoning models}}{20}{listing.132}\protected@file@percent }
\newlabel{lst:sys-prompt}{{D.1}{20}{System prompt for all reasoning models}{listing.132}{}}
\newlabel{lst:sys-prompt@cref}{{[listing][1][4]D.1}{[1][19][]20}{}{}{}}
\@writefile{lol}{\contentsline {listing}{\numberline {D.2}{\ignorespaces Prompt for masked frame prediction task}}{20}{listing.146}\protected@file@percent }
\newlabel{lst:mfp-prompt}{{D.2}{20}{Prompt for masked frame prediction task}{listing.146}{}}
\newlabel{lst:mfp-prompt@cref}{{[listing][2][4]D.2}{[1][19][]20}{}{}{}}
\@writefile{lol}{\contentsline {listing}{\numberline {D.3}{\ignorespaces Prompts for change detection task}}{21}{listing.165}\protected@file@percent }
\newlabel{lst:change-detection-prompt}{{D.3}{21}{Prompts for change detection task}{listing.165}{}}
\newlabel{lst:change-detection-prompt@cref}{{[listing][3][4]D.3}{[1][19][]21}{}{}{}}
\@writefile{lol}{\contentsline {listing}{\numberline {D.4}{\ignorespaces Prompts for planning task}}{22}{listing.179}\protected@file@percent }
\newlabel{lst:planning-prompt}{{D.4}{22}{Prompts for planning task}{listing.179}{}}
\newlabel{lst:planning-prompt@cref}{{[listing][4][4]D.4}{[1][19][]22}{}{}{}}
\BKM@entry{id=28,dest={617070656E6469782E313830},srcline={482}}{5C3337365C3337375C303030545C303030685C303030655C3030306F5C303030725C303030655C303030745C303030695C303030635C303030615C3030306C5C3030305C3034305C303030465C303030725C303030615C3030306D5C303030655C303030775C3030306F5C303030725C3030306B5C3030305C3034305C303030615C3030306E5C303030645C3030305C3034305C303030525C303030655C303030665C303030655C303030725C303030655C3030306E5C303030635C303030655C3030305C3034305C303030425C303030615C303030735C303030655C3030306C5C303030695C3030306E5C303030655C30303073}
\BKM@entry{id=29,dest={73756273656374696F6E2E313831},srcline={487}}{5C3337365C3337375C303030545C303030685C303030655C3030306F5C303030725C303030655C303030745C303030695C303030635C303030615C3030306C5C3030305C3034305C303030465C303030725C303030615C3030306D5C303030655C303030775C3030306F5C303030725C3030306B5C3030305C3034305C303030665C3030306F5C303030725C3030305C3034305C3030304E5C303030655C303030785C303030745C3030302D5C303030535C303030745C303030615C303030745C303030655C3030305C3034305C303030505C303030725C303030655C303030645C303030695C303030635C303030745C303030695C3030306F5C3030306E5C3030305C3034305C3030304D5C3030306F5C303030645C303030655C3030306C5C30303073}
\BKM@entry{id=30,dest={73756273756273656374696F6E2E313832},srcline={492}}{5C3337365C3337375C3030304E5C303030655C303030785C303030745C3030302D5C303030535C303030745C303030615C303030745C303030655C3030305C3034305C303030505C303030725C303030655C303030645C303030695C303030635C303030745C303030695C3030306F5C3030306E5C3030305C3034305C3030304D5C3030306F5C303030645C303030655C3030306C}
\BKM@entry{id=31,dest={73756273656374696F6E2E313838},srcline={534}}{5C3337365C3337375C3030304E5C3030306F5C3030306E5C3030302D5C3030304C5C3030304C5C3030304D5C3030305C3034305C303030425C303030615C303030735C303030655C3030306C5C303030695C3030306E5C303030655C3030305C3034305C303030415C303030675C303030655C3030306E5C303030745C30303073}
\BKM@entry{id=32,dest={73756273756273656374696F6E2E313839},srcline={539}}{5C3337365C3337375C303030415C303030755C303030745C303030755C3030306D5C3030306E5C3030302D5C303030535C303030695C3030306D5C303030755C3030306C5C303030615C303030745C3030306F5C303030725C3030305C3034305C303030415C303030675C303030655C3030306E5C30303074}
\citation{dreamerv3}
\@writefile{toc}{\contentsline {section}{\numberline {E}Theoretical Framework and Reference Baselines}{23}{appendix.180}\protected@file@percent }
\csxdef {autonum@sec:theoretical-frameworkReferenced}{}
\csxdef {autonum@sec:autumn-simulator-agentReferenced}{}
\csxdef {autonum@sec:random-agent-resultsReferenced}{}
\@writefile{toc}{\contentsline {subsection}{\numberline {E.1}Theoretical Framework for Next-State Prediction Models}{23}{subsection.181}\protected@file@percent }
\newlabel{sec:theoretical-framework}{{E.1}{23}{Final Normalized Perplexity}{subsection.181}{}}
\newlabel{sec:theoretical-framework@cref}{{[appendix][1][5]E.1}{[1][23][]23}{}{}{}}
\csxdef {autonum@sec:autumn-simulator-agentReferenced}{}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {E.1.1}Next-State Prediction Model}{23}{subsubsection.182}\protected@file@percent }
\newlabel{sec:next-state-prediction-model}{{E.1.1}{23}{Final Normalized Perplexity}{subsubsection.182}{}}
\newlabel{sec:next-state-prediction-model@cref}{{[subsubsection][1][5,1]E.1.1}{[1][23][]23}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {E.2}Non-LLM Baseline Agents}{23}{subsection.188}\protected@file@percent }
\newlabel{sec:baseline-agents}{{E.2}{23}{Final Normalized Perplexity}{subsection.188}{}}
\newlabel{sec:baseline-agents@cref}{{[appendix][2][5]E.2}{[1][23][]23}{}{}{}}
\csxdef {autonum@sec:autumn-simulator-agentReferenced}{}
\csxdef {autonum@sec:random-agent-resultsReferenced}{}
\BKM@entry{id=33,dest={73756273756273656374696F6E2E313930},srcline={556}}{5C3337365C3337375C303030525C303030615C3030306E5C303030645C3030306F5C3030306D5C3030302D5C303030415C303030675C303030655C3030306E5C303030745C3030305C3034305C303030425C303030615C303030735C303030655C3030306C5C303030695C3030306E5C30303065}
\BKM@entry{id=34,dest={617070656E6469782E313932},srcline={601}}{5C3337365C3337375C303030415C303030645C303030645C303030695C303030745C303030695C3030306F5C3030306E5C303030615C3030306C5C3030305C3034305C303030525C303030655C303030735C303030755C3030306C5C303030745C30303073}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {E.2.1}Autumn-Simulator Agent}{24}{subsubsection.189}\protected@file@percent }
\newlabel{sec:autumn-simulator-agent}{{E.2.1}{24}{Final Normalized Perplexity}{subsubsection.189}{}}
\newlabel{sec:autumn-simulator-agent@cref}{{[subsubsection][1][5,2]E.2.1}{[1][23][]24}{}{}{}}
\@writefile{toc}{\contentsline {paragraph}{Task-specific solvers.}{24}{subsubsection.189}\protected@file@percent }
\@writefile{toc}{\contentsline {subsubsection}{\numberline {E.2.2}Random-Agent Baseline}{24}{subsubsection.190}\protected@file@percent }
\newlabel{sec:random-agent-results}{{E.2.2}{24}{Final Normalized Perplexity}{subsubsection.190}{}}
\newlabel{sec:random-agent-results@cref}{{[subsubsection][2][5,2]E.2.2}{[1][24][]24}{}{}{}}
\csxdef {autonum@tab:random_agent_probabilitiesReferenced}{}
\@writefile{lot}{\contentsline {table}{\numberline {E.1}{\ignorespaces Random-agent baseline by environment. Environments 1--26 are deterministic; 27--43 are stochastic. Columns report the probability of triggering the change within 1000 timesteps (CD) and reaching the goal within 1000 timesteps (PL).}}{24}{table.caption.191}\protected@file@percent }
\newlabel{tab:random_agent_probabilities}{{E.1}{24}{Random-agent baseline by environment. Environments 1--26 are deterministic; 27--43 are stochastic. Columns report the probability of triggering the change within 1000 timesteps (CD) and reaching the goal within 1000 timesteps (PL)}{table.caption.191}{}}
\newlabel{tab:random_agent_probabilities@cref}{{[table][1][5]E.1}{[1][24][]24}{}{}{}}
\BKM@entry{id=35,dest={73756273656374696F6E2E313933},srcline={609}}{5C3337365C3337375C303030445C303030655C303030745C303030615C303030695C3030306C5C303030655C303030645C3030305C3034305C303030505C303030655C303030725C303030665C3030306F5C303030725C3030306D5C303030615C3030306E5C303030635C303030655C3030305C3034305C303030415C3030306E5C303030615C3030306C5C303030795C303030735C303030695C30303073}
\BKM@entry{id=36,dest={73756273756273656374696F6E2E313934},srcline={614}}{5C3337365C3337375C303030505C303030655C303030725C3030302D5C303030455C3030306E5C303030765C303030695C303030725C3030306F5C3030306E5C3030306D5C303030655C3030306E5C303030745C3030305C3034305C303030535C303030635C3030306F5C303030725C303030655C30303073}
\BKM@entry{id=37,dest={73756273756273656374696F6E2E313935},srcline={625}}{5C3337365C3337375C303030505C303030725C3030306F5C3030306D5C303030705C303030745C3030305C3034305C303030525C3030306F5C303030625C303030755C303030735C303030745C3030306E5C303030655C303030735C303030735C3030305C3034305C303030415C3030306E5C303030615C3030306C5C303030795C303030735C303030695C30303073}
\citation{autumnbench_dataset}
\BKM@entry{id=38,dest={73756273756273656374696F6E2E313938},srcline={652}}{5C3337365C3337375C303030505C303030655C303030725C303030665C3030306F5C303030725C3030306D5C303030615C3030306E5C303030635C303030655C3030305C3034305C303030765C303030655C303030725C303030735C303030755C303030735C3030305C3034305C303030435C3030306F5C3030306D5C303030705C303030755C303030745C303030615C303030745C303030695C3030306F5C3030306E5C303030615C3030306C5C3030305C3034305C303030435C3030306F5C303030735C30303074}
\@writefile{toc}{\contentsline {section}{\numberline {F}Additional Results}{25}{appendix.192}\protected@file@percent }
\newlabel{sec:additional_results}{{F}{25}{Final Normalized Perplexity}{appendix.192}{}}
\newlabel{sec:additional_results@cref}{{[appendix][6][]F}{[1][24][]25}{}{}{}}
\csxdef {autonum@sec:detailed-performanceReferenced}{}
\csxdef {autonum@sec:behavioral-analysisReferenced}{}
\csxdef {autonum@sec:context-usageReferenced}{}
\csxdef {autonum@sec:external-correlationsReferenced}{}
\csxdef {autonum@sec:qualitative-examplesReferenced}{}
\@writefile{toc}{\contentsline {subsection}{\numberline {F.1}Detailed Performance Analysis}{25}{subsection.193}\protected@file@percent }
\newlabel{sec:detailed-performance}{{F.1}{25}{Final Normalized Perplexity}{subsection.193}{}}
\newlabel{sec:detailed-performance@cref}{{[appendix][1][6]F.1}{[1][25][]25}{}{}{}}
\csxdef {autonum@sec:per-env-scoresReferenced}{}
\csxdef {autonum@sec:cost-performanceReferenced}{}
\csxdef {autonum@sec:prompt-robustnessReferenced}{}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {F.1.1}Per-Environment Scores}{25}{subsubsection.194}\protected@file@percent }
\newlabel{sec:per-env-scores}{{F.1.1}{25}{Final Normalized Perplexity}{subsubsection.194}{}}
\newlabel{sec:per-env-scores@cref}{{[subsubsection][1][6,1]F.1.1}{[1][25][]25}{}{}{}}
\csxdef {autonum@tab:avg_scoresReferenced}{}
\@writefile{toc}{\contentsline {paragraph}{Saturation check with Claude~Opus~4.6.}{25}{subsubsection.194}\protected@file@percent }
\csxdef {autonum@tab:avg_scoresReferenced}{}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {F.1.2}Prompt Robustness Analysis}{25}{subsubsection.195}\protected@file@percent }
\newlabel{sec:prompt-robustness}{{F.1.2}{25}{Final Normalized Perplexity}{subsubsection.195}{}}
\newlabel{sec:prompt-robustness@cref}{{[subsubsection][2][6,1]F.1.2}{[1][25][]25}{}{}{}}
\@writefile{lot}{\contentsline {table}{\numberline {F.1}{\ignorespaces Performance of reasoning models under different prompts on a subset of AutumnBench problems}}{25}{table.caption.196}\protected@file@percent }
\newlabel{tab:prompt_comparison_subset}{{F.1}{25}{Performance of reasoning models under different prompts on a subset of AutumnBench problems}{table.caption.196}{}}
\newlabel{tab:prompt_comparison_subset@cref}{{[table][1][6]F.1}{[1][25][]25}{}{}{}}
\csxdef {autonum@tab:prompt_comparison_subsetReferenced}{}
\BKM@entry{id=39,dest={73756273656374696F6E2E323030},srcline={731}}{5C3337365C3337375C303030425C303030655C303030685C303030615C303030765C303030695C3030306F5C303030725C303030615C3030306C5C3030305C3034305C303030415C3030306E5C303030615C3030306C5C303030795C303030735C303030695C30303073}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {F.1.3}Performance versus Computational Cost}{26}{subsubsection.198}\protected@file@percent }
\newlabel{sec:cost-performance}{{F.1.3}{26}{Final Normalized Perplexity}{subsubsection.198}{}}
\newlabel{sec:cost-performance@cref}{{[subsubsection][3][6,1]F.1.3}{[1][25][]26}{}{}{}}
\@writefile{toc}{\contentsline {paragraph}{Overall findings.}{26}{subsubsection.198}\protected@file@percent }
\@writefile{toc}{\contentsline {paragraph}{Task-specific patterns.}{26}{subsubsection.198}\protected@file@percent }
\@writefile{toc}{\contentsline {paragraph}{Environment characteristics.}{26}{subsubsection.198}\protected@file@percent }
\csxdef {autonum@tab:random_agent_probabilitiesReferenced}{}
\@writefile{lot}{\contentsline {table}{\numberline {F.2}{\ignorespaces Average scores by environment across three task types and agents. Qwen refers to Qwen3-235B-A22B-Thinking-2507.}}{26}{table.caption.199}\protected@file@percent }
\newlabel{tab:avg_scores}{{F.2}{26}{Average scores by environment across three task types and agents. Qwen refers to Qwen3-235B-A22B-Thinking-2507}{table.caption.199}{}}
\newlabel{tab:avg_scores@cref}{{[table][2][6]F.2}{[1][26][]26}{}{}{}}
\BKM@entry{id=40,dest={73756273756273656374696F6E2E323031},srcline={736}}{5C3337365C3337375C303030415C303030635C303030745C303030695C3030306F5C3030306E5C3030302D5C303030445C303030695C303030735C303030745C303030725C303030695C303030625C303030755C303030745C303030695C3030306F5C3030306E5C3030305C3034305C303030415C3030306E5C303030615C3030306C5C303030795C303030735C303030695C30303073}
\BKM@entry{id=41,dest={73756273756273656374696F6E2E323033},srcline={805}}{5C3337365C3337375C3030304F5C3030306E5C3030302D5C303030435C3030306C5C303030615C303030755C303030735C303030655C3030305C3034305C303030435C3030306F5C303030765C303030655C303030725C303030615C303030675C30303065}
\@writefile{toc}{\contentsline {subsection}{\numberline {F.2}Behavioral Analysis}{27}{subsection.200}\protected@file@percent }
\newlabel{sec:behavioral-analysis}{{F.2}{27}{Final Normalized Perplexity}{subsection.200}{}}
\newlabel{sec:behavioral-analysis@cref}{{[appendix][2][6]F.2}{[1][26][]27}{}{}{}}
\csxdef {autonum@sec:resultsReferenced}{}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {F.2.1}Action-Distribution Analysis}{27}{subsubsection.201}\protected@file@percent }
\newlabel{sec:action-distribution}{{F.2.1}{27}{Final Normalized Perplexity}{subsubsection.201}{}}
\newlabel{sec:action-distribution@cref}{{[subsubsection][1][6,2]F.2.1}{[1][27][]27}{}{}{}}
\@writefile{lot}{\contentsline {table}{\numberline {F.3}{\ignorespaces Unique clicks and directional actions by environment and agent. Qwen refers to Qwen3-235B-A22B-Thinking-2507.}}{27}{table.caption.202}\protected@file@percent }
\newlabel{tab:avg_actions}{{F.3}{27}{Unique clicks and directional actions by environment and agent. Qwen refers to Qwen3-235B-A22B-Thinking-2507}{table.caption.202}{}}
\newlabel{tab:avg_actions@cref}{{[table][3][6]F.3}{[1][27][]27}{}{}{}}
\csxdef {autonum@tab:avg_actionsReferenced}{}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {F.2.2}On-Clause Coverage}{27}{subsubsection.203}\protected@file@percent }
\newlabel{sec:coverage}{{F.2.2}{27}{Final Normalized Perplexity}{subsubsection.203}{}}
\newlabel{sec:coverage@cref}{{[subsubsection][2][6,2]F.2.2}{[1][27][]27}{}{}{}}
\BKM@entry{id=42,dest={73756273756273656374696F6E2E323034},srcline={812}}{5C3337365C3337375C303030525C303030655C303030735C303030655C303030745C3030305C3034305C303030535C303030655C303030715C303030755C303030655C3030306E5C303030635C303030655C3030305C3034305C303030415C3030306E5C303030615C3030306C5C303030795C303030735C303030695C30303073}
\citation{coenen2015strategies,bramley2018intuitive}
\BKM@entry{id=43,dest={73756273756273656374696F6E2E323036},srcline={842}}{5C3337365C3337375C303030435C3030306F5C3030306E5C303030745C303030655C303030785C303030745C3030302D5C3030304C5C303030655C3030306E5C303030675C303030745C303030685C3030305C3034305C303030535C303030635C303030615C3030306C5C303030695C3030306E5C30303067}
\citation{wang2026context}
\BKM@entry{id=44,dest={73756273656374696F6E2E323037},srcline={847}}{5C3337365C3337375C303030435C3030306F5C3030306E5C303030745C303030655C303030785C303030745C3030305C3034305C303030555C303030735C303030615C303030675C303030655C3030305C3034305C303030415C3030306E5C303030615C3030306C5C303030795C303030735C303030695C30303073}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {F.2.3}Reset Sequence Analysis}{28}{subsubsection.204}\protected@file@percent }
\newlabel{sec:lcs-analysis}{{F.2.3}{28}{Final Normalized Perplexity}{subsubsection.204}{}}
\newlabel{sec:lcs-analysis@cref}{{[subsubsection][3][6,2]F.2.3}{[1][28][]28}{}{}{}}
\@writefile{lot}{\contentsline {table}{\numberline {F.4}{\ignorespaces LCS ratio between pre- and post-reset action sequences with adaptive windows sized to $6\%$ of interaction length, clipped to $[10, 50]$ actions. Higher values indicate more structured resets. All human--model differences significant at $p<10^{-18}$ under the Mann--Whitney U test.}}{28}{table.caption.205}\protected@file@percent }
\newlabel{tab:lcs_ratio}{{F.4}{28}{LCS ratio between pre- and post-reset action sequences with adaptive windows sized to $6\%$ of interaction length, clipped to $[10, 50]$ actions. Higher values indicate more structured resets. All human--model differences significant at $p<10^{-18}$ under the Mann--Whitney U test}{table.caption.205}{}}
\newlabel{tab:lcs_ratio@cref}{{[table][4][6]F.4}{[1][28][]28}{}{}{}}
\csxdef {autonum@tab:lcs_ratioReferenced}{}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {F.2.4}Context-Length Scaling}{28}{subsubsection.206}\protected@file@percent }
\newlabel{sec:context-scaling}{{F.2.4}{28}{Final Normalized Perplexity}{subsubsection.206}{}}
\newlabel{sec:context-scaling@cref}{{[subsubsection][4][6,2]F.2.4}{[1][28][]28}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {F.3}Context Usage Analysis}{28}{subsection.207}\protected@file@percent }
\newlabel{sec:context-usage}{{F.3}{28}{Final Normalized Perplexity}{subsection.207}{}}
\newlabel{sec:context-usage@cref}{{[appendix][3][6]F.3}{[1][28][]28}{}{}{}}
\csxdef {autonum@tab:context_usageReferenced}{}
\@writefile{lot}{\contentsline {table}{\numberline {F.5}{\ignorespaces Context usage per model. We measure tokens at the final test-phase turn, which includes the complete interaction history.}}{28}{table.caption.208}\protected@file@percent }
\newlabel{tab:context_usage}{{F.5}{28}{Context usage per model. We measure tokens at the final test-phase turn, which includes the complete interaction history}{table.caption.208}{}}
\newlabel{tab:context_usage@cref}{{[table][5][6]F.5}{[1][28][]28}{}{}{}}
\BKM@entry{id=45,dest={73756273656374696F6E2E323039},srcline={876}}{5C3337365C3337375C303030435C3030306F5C303030725C303030725C303030655C3030306C5C303030615C303030745C303030695C3030306F5C3030306E5C3030305C3034305C303030775C303030695C303030745C303030685C3030305C3034305C303030455C303030785C303030745C303030655C303030725C3030306E5C303030615C3030306C5C3030305C3034305C303030425C303030655C3030306E5C303030635C303030685C3030306D5C303030615C303030725C3030306B5C30303073}
\citation{li24simpler}
\citation{jimenez2024swebench}
\citation{terminalbench}
\citation{rein2024gpqa}
\BKM@entry{id=46,dest={73756273656374696F6E2E323131},srcline={911}}{5C3337365C3337375C303030515C303030755C303030615C3030306C5C303030695C303030745C303030615C303030745C303030695C303030765C303030655C3030305C3034305C303030455C303030785C303030615C3030306D5C303030705C3030306C5C303030655C30303073}
\@writefile{toc}{\contentsline {subsection}{\numberline {F.4}Correlation with External Benchmarks}{29}{subsection.209}\protected@file@percent }
\newlabel{sec:external-correlations}{{F.4}{29}{Final Normalized Perplexity}{subsection.209}{}}
\newlabel{sec:external-correlations@cref}{{[appendix][4][6]F.4}{[1][29][]29}{}{}{}}
\csxdef {autonum@tab:external_correlationsReferenced}{}
\@writefile{lot}{\contentsline {table}{\numberline {F.6}{\ignorespaces AutumnBench scores alongside external benchmark scores, with Spearman $\rho $ correlations. \textsuperscript  {*}$p < 0.05$, \textsuperscript  {**}$p < 0.001$.}}{29}{table.caption.210}\protected@file@percent }
\newlabel{tab:external_correlations}{{F.6}{29}{AutumnBench scores alongside external benchmark scores, with Spearman $\rho $ correlations. \textsuperscript {*}$p < 0.05$, \textsuperscript {**}$p < 0.001$}{table.caption.210}{}}
\newlabel{tab:external_correlations@cref}{{[table][6][6]F.6}{[1][29][]29}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {F.5}Qualitative Examples}{29}{subsection.211}\protected@file@percent }
\newlabel{sec:qualitative-examples}{{F.5}{29}{Final Normalized Perplexity}{subsection.211}{}}
\newlabel{sec:qualitative-examples@cref}{{[appendix][5][6]F.5}{[1][29][]29}{}{}{}}
\csxdef {autonum@lst:mfp-promptReferenced}{}
\csxdef {autonum@lst:change-detection-promptReferenced}{}
\csxdef {autonum@lst:planning-promptReferenced}{}
\csxdef {autonum@lst:example_scratchpadReferenced}{}
\csxdef {autonum@lst:mfp_choicesReferenced}{}
\@writefile{lol}{\contentsline {lstlisting}{tables/scratchpad\textunderscore \textunderscore claude\textunderscore mfp\textunderscore exp\textunderscore particles.txt}{30}{lstlisting.212}\protected@file@percent }
\@writefile{lol}{\contentsline {listing}{\numberline {F.1}{\ignorespaces Example scratchpad for the \obfsname  {exp\_particles} environment, with choices listed in \autonum@processReference {autonum@referenceCrefOld}{forcsvlist}{lst:mfp_choices}.}}{33}{listing.463}\protected@file@percent }
\csxdef {autonum@lst:mfp_choicesReferenced}{}
\newlabel{lst:example_scratchpad}{{F.1}{33}{Example scratchpad for the \obfsname {exp\_particles} environment, with choices listed in \Cref {lst:mfp_choices}}{listing.463}{}}
\newlabel{lst:example_scratchpad@cref}{{[listing][1][6]F.1}{[1][33][]33}{}{}{}}
\@writefile{lol}{\contentsline {listing}{\numberline {F.2}{\ignorespaces Answer choices, indexed 0--5, supplied for masked frame prediction in the \obfsname  {exp\_particles} environment.}}{34}{listing.521}\protected@file@percent }
\newlabel{lst:mfp_choices}{{F.2}{34}{Answer choices, indexed 0--5, supplied for masked frame prediction in the \obfsname {exp\_particles} environment}{listing.521}{}}
\newlabel{lst:mfp_choices@cref}{{[listing][2][6]F.2}{[1][33][]34}{}{}{}}
\gdef \@abspage@last{34}
\end{filecontents}


==> new_plots/init_plot/interaction_phase.tex <==
% Interaction phase diagram: two boxes and two labeled arrows (CURVED VERSION)
% This is a fragment intended to be \subimport'ed or \input into a tikzpicture
% Requires the caller to load: \usetikzlibrary{arrows.meta,calc}

% Local styles
\tikzset{
  ip/box/.style={draw, rounded corners=6pt, minimum width=4.2cm, minimum height=3.0cm, line width=0.8pt, align=center, font=\large},
  ip/arrow/.style={->, line width=0.9pt},
  ip/label/.style={font=\normalsize, fill=white, inner sep=2pt, rounded corners=2pt},
  % Outer framing styles (match test phase look)
  ip/outerbox/.style={draw=black, rounded corners=8pt, line width=0.8pt},
  ip/title/.style={font=\large\bfseries, text=black}
}

% Browser header configuration (shared with test phase)
\providecommand{\BrowserBarH}{0.5cm}
\providecommand{\BrowserBarAddrTop}{0.12cm}
\providecommand{\BrowserBarAddrBottomPad}{0.12cm}
\providecommand{\IPButtonLabelFont}{\tiny}

% Soft background colors for boxes
\colorlet{IPLeftBg}{blue!22}
\colorlet{IPRightBg}{red!30!brown!35}

% Coordinate system (units in cm)
\begin{scope}[x=1cm,y=1cm]

  % Title drawn later relative to content bounds

  % Boxes
  % Left/top: drawless container, then render stacked grids inside it
  % Place stacked frames above the agent (vertical layout)
  % Positioned to start from origin area
  \node[ip/box, draw=none, inner sep=0pt] (stack) at (2.1,4.5) {};
  % Clip to the box extents (min size 4.2cm x 3.0cm)
  \begin{scope}
    % Background to simulate browser content area
    \path[fill=black!5]
    ([xshift=-2.1cm,yshift=-2.0cm]stack.center)
    rectangle
    ([xshift= 2.1cm,yshift= 1.5cm]stack.center);
    % Center and scale the stacked grids fragment inside the box
    % Apply an unscaled offset to center the fragment's bounding box
    \def\cellsz{0.35cm}
    \begin{scope}[shift={(stack.center)}]
      \begin{scope}[shift={(-0.85,-1.15)}]
        \begin{scope}[scale=1]
          \subimport{.}{stacked_treasure.tex}

          \begin{scope}[shift={(0.2,0.0)}]

            \begin{scope}[x=\cellsz, y=\cellsz, line cap=round, line join=round]

              \def\btnYlow{-2}
              \def\btnYhigh{-1}

              % derive button height and font size as a fraction of grid cell size
              \pgfmathsetmacro{\btnHeight}{\btnYhigh-\btnYlow}
              \pgfmathsetlengthmacro{\btnFont}{0.55*\btnHeight*\cellsz}
              \pgfmathsetlengthmacro{\btnFontBaseline}{1.1*\btnFont}
              % text widths to keep labels inside outlines
              \pgfmathsetlengthmacro{\btnTextWidthLeft}{2.2*\cellsz}
              \pgfmathsetlengthmacro{\btnTextWidthRight}{3.2*\cellsz}
              % Reset button
              \node[
              draw=\maraGridBorderColor,
              fill=black!40,
              rounded corners=\maraBorderRadius,
              inner sep=0pt,
              fit={(-0.5,\btnYlow) (2,\btnYhigh)},
              label={[font=\IPButtonLabelFont,text=black,align=center]center:{Reset}}
              ] (IPResetButton) {};
              % Go to Test button
              \node[
              draw=\maraGridBorderColor,
              fill=black!40,
              rounded corners=\maraBorderRadius,
              inner sep=0pt,
              fit={(2.5,\btnYlow) (6.0,\btnYhigh)},
              label={[font=\IPButtonLabelFont,text=black,align=center]center:{Go to Test}}
              ] (IPUIButton) {};
            \end{scope}
          \end{scope}
        \end{scope}
      \end{scope}
    \end{scope}
  \end{scope}
  % (Browser header removed)
  % Agent and interaction arrows are drawn by the parent diagram


\end{scope}


==> new_plots/init_plot/pic_human_icon.tex <==
% Human icon pic definition (from test/test.tex illustration)
% Usage: \pic (name) at (x,y) {human_icon};
\tikzset{
    pics/human_icon/.style={code={%
                    \begin{scope}[y=1cm, x=1cm, inner sep=0pt, outer sep=0pt]
                        \def \globalscale {1.000000}
                        \begin{scope}[yscale=\globalscale,xscale=\globalscale, every node/.append style={scale=\globalscale}]
                            % Translate so the illustration's center is at the origin
                            \begin{scope}[shift={(-12.945, -93)}]
                                \path[fill,shift={(0,54.186666666666675)},scale=2.0] (7.5707, 24.9334).. controls (7.7914, 25.1749) and (8.1229, 25.2749) .. (8.4425, 25.2838).. controls (8.7652, 25.2967) and (9.103, 25.1567) .. (9.3336, 24.9334).. controls (10.1875, 25.051) and (10.858, 24.5093) .. (10.9007, 23.6371).. controls (11.4577, 23.2429) and (11.4979, 22.3437) .. (11.0841, 21.8259).. controls (11.0228, 21.7491) and (10.9513, 21.6791) .. (10.8832, 21.6083).. controls (10.9195, 21.1444) and (10.6106, 20.6804) .. (10.2105, 20.4685).. controls (9.91, 20.3094) and (9.6816, 20.3285) .. (9.3566, 20.3269).. controls (9.1071, 20.182) and (9.0865, 20.0527) .. (8.7192, 19.9777).. controls (8.7324, 19.4274) and (8.5849, 18.8305) .. (8.273, 18.3725).. controls (8.1592, 18.2054) and (8.0127, 18.0691) .. (7.9123, 17.8914).. controls (7.5531, 17.2557) and (7.7863, 16.4041) .. (8.0641, 15.7725).. controls (8.1297, 15.6233) and (8.2863, 15.3971) .. (8.0328, 15.3375).. controls (7.8237, 15.3862) and (7.6892, 15.9535) .. (7.6272, 16.1495).. controls (7.4166, 16.8157) and (7.3371, 17.4989) .. (7.7267, 18.1203).. controls (7.8478, 18.3135) and (8.0019, 18.4455) .. (8.119, 18.6551).. controls (8.343, 19.0564) and (8.4238, 19.4982) .. (8.4425, 19.9527).. controls (7.9826, 19.9736) and (7.9019, 20.1002) .. (7.5795, 20.3209) -- (7.5707, 20.3269).. controls (7.0583, 20.3854) and (7.0065, 20.2614) .. (6.4783, 20.6303) -- (6.4759, 20.6177).. controls (6.3572, 20.0439) and (5.5977, 19.8771) .. (5.2752, 20.3892).. controls (4.9547, 20.898) and (5.3963, 21.5133) .. (6.0444, 21.3567).. controls (6.0276, 21.4405) and (6.0144, 21.5235) .. (6.0037, 21.6083).. controls (5.6685, 21.9176) and (5.5215, 22.2779) .. (5.523, 22.7345).. controls (5.1957, 22.754) and (4.8825, 22.7024) .. (4.574, 22.5951).. controls (3.6767, 22.2558) and (3.0958, 21.4364) .. (3.0699, 20.475).. controls (3.0573, 20.0031) and (3.1086, 20.1688) .. (2.9005, 19.7321) -- (2.5937, 19.0831).. controls (2.5584, 19.0081) and (2.4498, 18.8389) .. (2.4628, 18.7554).. controls (2.4867, 18.602) and (2.9072, 18.6557) .. (3.0271, 18.5632).. controls (3.1086, 18.5003) and (3.0783, 18.3581) .. (3.0785, 18.2693) -- (3.0776, 17.7865).. controls (3.0755, 16.4785) and (4.0466, 17.2523) .. (4.6207, 16.806).. controls (4.8008, 16.666) and (4.9071, 16.4774) .. (4.9354, 16.2529) -- (5.5963, 16.2523).. controls (5.7169, 16.2526) and (6.0365, 16.3104) .. (6.0465, 16.1215).. controls (6.0575, 15.9135) and (5.7582, 15.9705) .. (5.6343, 15.9706) -- (4.9354, 15.971).. controls (4.9338, 15.8209) and (4.9979, 15.3545) .. (4.8062, 15.3516).. controls (4.7361, 15.3505) and (4.6925, 15.3859) .. (4.6453, 15.4324).. controls (4.6383, 15.5038) and (4.6444, 15.5809) .. (4.6447, 15.653) -- (4.6473, 16.1349).. controls (4.6471, 16.2696) and (4.6211, 16.3879) .. (4.537, 16.4963).. controls (4.2095, 16.9181) and (3.5638, 16.4335) .. (3.0528, 16.9488).. controls (2.7889, 17.215) and (2.7972, 17.4815) .. (2.7974, 17.8276) -- (2.7978, 18.3372).. controls (2.2025, 18.422) and (2.0443, 18.5777) .. (2.3261, 19.1671).. controls (2.4199, 19.3633) and (2.5068, 19.5629) .. (2.6008, 19.7591).. controls (2.8285, 20.2344) and (2.7841, 20.0572) .. (2.7941, 20.5702).. controls (2.8175, 21.7846) and (3.8523, 22.8678) .. (5.0491, 22.9958).. controls (5.2242, 23.0145) and (5.3969, 23.0098) .. (5.5726, 23.0063).. controls (5.6544, 23.2547) and (5.7987, 23.4735) .. (6.0037, 23.6371).. controls (6.0474, 24.4573) and (6.7281, 25.1377) .. (7.5707, 24.9334) -- cycle(8.3708, 25.0006).. controls (8.1704, 24.98) and (7.9635, 24.9074) .. (7.8101, 24.7727).. controls (7.7622, 24.7305) and (7.7208, 24.6688) .. (7.6675, 24.6348) -- (7.6574, 24.6357).. controls (7.5742, 24.6432) and (7.494, 24.6679) .. (7.411, 24.6762).. controls (6.8513, 24.7317) and (6.3372, 24.3114) .. (6.2873, 23.7495).. controls (6.2804, 23.6719) and (6.2854, 23.5942) .. (6.2824, 23.5166).. controls (6.2174, 23.4546) and (6.1438, 23.4022) .. (6.0807, 23.3383).. controls (5.707, 22.9598) and (5.7082, 22.2989) .. (6.0787, 21.9181).. controls (6.3918, 21.5964) and (6.2085, 21.7972) .. (6.318, 21.3954).. controls (6.4558, 20.89) and (6.9241, 20.5375) .. (7.4535, 20.6092).. controls (7.734, 20.6473) and (7.6548, 20.6282) .. (7.8302, 20.4691).. controls (8.0334, 20.2849) and (8.28, 20.2299) .. (8.5449, 20.2345).. controls (9.0447, 20.3027) and (8.9926, 20.4875) .. (9.2481, 20.6303) -- (9.2582, 20.6307).. controls (9.3573, 20.6344) and (9.4558, 20.6088) .. (9.5547, 20.6043).. controls (10.1098, 20.5794) and (10.5871, 20.9916) .. (10.6049, 21.5527).. controls (10.6124, 21.7881) and (10.6085, 21.7319) .. (10.7754, 21.8914).. controls (11.1953, 22.2924) and (11.1941, 22.9954) .. (10.7648, 23.39).. controls (10.7168, 23.4342) and (10.6633, 23.4719) .. (10.6158, 23.5166).. controls (10.619, 24.1427) and (10.2518, 24.6799) .. (9.5882, 24.6824).. controls (9.4318, 24.683) and (9.2939, 24.5789) .. (9.171, 24.6998).. controls (8.9732, 24.8943) and (8.6559, 25.0488) .. (8.3708, 25.0006) -- cycle(5.7612, 21.1058).. controls (5.2782, 21.0029) and (5.3955, 20.3003) .. (5.9002, 20.3606).. controls (6.3673, 20.4749) and (6.2783, 21.1549) .. (5.7612, 21.1058) -- cycle;

                                \path[fill=lightbulb,shift={(0,54.186666666666675)},scale=2.0] (8.4898, 23.8205).. controls (8.2267, 23.8008) and (8.2357, 24.1173) .. (8.4002, 24.1889).. controls (8.6022, 24.1999) and (8.6388, 23.9047) .. (8.4898, 23.8205) -- cycle;

                                \path[fill=lightbulb,shift={(0,54.186666666666675)},scale=2.0] (7.6675, 23.488).. controls (7.5029, 23.4816) and (7.2771, 23.7975) .. (7.5238, 23.8588).. controls (7.6785, 23.8706) and (7.8994, 23.6177) .. (7.6675, 23.488) -- cycle;

                                \path[fill=lightbulb,shift={(0,54.186666666666675)},scale=2.0] (9.2481, 23.488).. controls (8.9647, 23.4878) and (9.0873, 23.7519) .. (9.2812, 23.8588).. controls (9.5569, 23.874) and (9.4189, 23.5528) .. (9.2481, 23.488) -- cycle;

                                % Main bulb shape (filled), drawn without stroke
                                \path[fill=lightbulb, draw=none, shift={(0,54.186666666666675)},scale=2.0]
                                (8.4425, 21.0532).. controls (7.7309, 21.0468) and (8.0062, 21.4587) .. (7.8859, 21.8567).. controls (7.8567, 21.9531) and (7.799, 22.0152) .. (7.7355, 22.0906).. controls (7.2081, 22.7176) and (7.6005, 23.6157) .. (8.4002, 23.6708).. controls (8.9134, 23.7131) and (9.3311, 23.2502) .. (9.3378, 22.759).. controls (9.3452, 22.2163) and (9.007, 22.1361) .. (8.9561, 21.8248).. controls (8.8887, 21.4125) and (9.0938, 21.0459) .. (8.4425, 21.0532) -- cycle;

                                \path[fill=lightbulb,shift={(0,54.186666666666675)},scale=2.0] (8.4425, 21.0532).. controls (7.7309, 21.0468) and (8.0062, 21.4587) .. (7.8859, 21.8567).. controls (7.8567, 21.9531) and (7.799, 22.0152) .. (7.7355, 22.0906).. controls (7.2081, 22.7176) and (7.6005, 23.6157) .. (8.4002, 23.6708).. controls (8.9134, 23.7131) and (9.3311, 23.2502) .. (9.3378, 22.759).. controls (9.3452, 22.2163) and (9.007, 22.1361) .. (8.9561, 21.8248).. controls (8.8887, 21.4125) and (9.0938, 21.0459) .. (8.4425, 21.0532) -- cycle(8.3708, 23.3935).. controls (7.8169, 23.3266) and (7.5758, 22.6886) .. (7.9411, 22.2633).. controls (8.0703, 22.1129) and (8.1149, 22.0102) .. (8.1845, 21.8219) -- (8.4898, 21.8219) -- (8.6778, 21.8219).. controls (8.7177, 22.0534) and (8.8055, 22.1613) .. (8.9404, 22.3422).. controls (9.275, 22.7911) and (8.9008, 23.4878) .. (8.3708, 23.3935) -- cycle(8.1845, 21.5498).. controls (8.1842, 21.4998) and (8.1733, 21.4019) .. (8.2097, 21.3635).. controls (8.2727, 21.297) and (8.5507, 21.3041) .. (8.6406, 21.3567).. controls (8.6855, 21.4093) and (8.6765, 21.4843) .. (8.6778, 21.5498) -- (8.1845, 21.5498) -- cycle;

                                \path[fill=lightbulb,shift={(0,54.186666666666675)},scale=2.0] (7.2755, 22.7663).. controls (6.791, 22.7425) and (6.9313, 23.0112) .. (7.0651, 23.0263).. controls (7.1402, 23.0301) and (7.2361, 23.0431) .. (7.3075, 23.0167).. controls (7.4419, 22.967) and (7.3906, 22.8007) .. (7.2755, 22.7663) -- cycle;

                                \path[fill=lightbulb,shift={(0,54.186666666666675)},scale=2.0] (9.7884, 22.7663).. controls (9.7129, 22.7653) and (9.6093, 22.7518) .. (9.5377, 22.7769).. controls (9.4042, 22.8239) and (9.4324, 22.9787) .. (9.5456, 23.0263).. controls (9.6253, 23.0275) and (9.7254, 23.0398) .. (9.8011, 23.0128).. controls (9.9292, 22.9671) and (9.9024, 22.8064) .. (9.7884, 22.7663) -- cycle;

                                \path[fill,shift={(0,54.186666666666675)},scale=2.0] (4.615, 19.6981).. controls (3.9383, 19.6794) and (3.8467, 20.6855) .. (4.574, 20.7339).. controls (5.2178, 20.7355) and (5.2904, 19.7874) .. (4.615, 19.6981) -- cycle(4.5427, 20.4581).. controls (4.2476, 20.3627) and (4.2789, 19.9871) .. (4.615, 19.9777).. controls (4.9203, 20.062) and (4.8546, 20.4863) .. (4.5427, 20.4581) -- cycle;
                            \end{scope}
                        \end{scope}
                    \end{scope}
                }}
}


==> new_plots/init_plot/pic_llm_icon.tex <==
% AI icon pic definition (rewritten to use plotting code from test/test.tex)

\providecommand{\llmIconAIFont}{\sffamily\bfseries\large}
\providecommand{\llmIconAIColor}{black}

\tikzset{
    pics/llm_icon/.style={code={%
                    \begin{scope}[y=1cm, x=1cm, inner sep=0pt, outer sep=0pt]
                        % Keep the same scaling approach as test/test.tex
                        \def \globalscale {1.00000}
                        \begin{scope}[yscale=\globalscale,xscale=\globalscale, every node/.append style={scale=\globalscale}]
                            % Translate so the illustration's center is at the origin
                            \begin{scope}[shift={(-41.073, 40.36605)}]
                                % \path[fill=white] (2.1077, -1.242) rectangle (80.0383, -79.4901);
                                % Colored sparkles to represent LLM variants (Gemini-like palette)
                                \definecolor{GemColorA}{RGB}{251,200,5}%{66,133,244}  % blue
                                \definecolor{GemColorB}{RGB}{251,200,5}%{52,168,83}   % green
                                \definecolor{GemColorC}{RGB}{251,200,5}%{251,188,5}   % yellow
                                \definecolor{GemColorD}{RGB}{0,0,0}%{100,122,233}
                                \path[fill=GemColorD] (61.8686, -41.3684).. controls (61.8546, -41.7788) and (61.8479, -42.1894) .. (61.8247, -42.599).. controls (61.8046, -42.9538) and (61.7712, -43.3078) .. (61.7334, -43.6613).. controls (61.6977, -43.9933) and (61.6522, -44.3246) .. (61.6045, -44.6553).. controls (61.5156, -45.2713) and (61.3899, -45.8801) .. (61.2397, -46.4839).. controls (60.8777, -47.9385) and (60.3634, -49.3374) .. (59.6934, -50.6786).. controls (58.8505, -52.3661) and (57.7964, -53.9099) .. (56.5288, -55.3069).. controls (54.7796, -57.2347) and (52.7399, -58.7798) .. (50.4103, -59.9406).. controls (49.0498, -60.6184) and (47.6303, -61.1378) .. (46.1534, -61.4987).. controls (45.5613, -61.6434) and (44.9646, -61.7633) .. (44.3619, -61.8551).. controls (43.9478, -61.9181) and (43.5322, -61.9683) .. (43.1152, -62.0085).. controls (42.2503, -62.0922) and (41.3837, -62.1202) .. (40.5156, -62.0969).. controls (40.0883, -62.0855) and (39.6616, -62.0607) .. (39.2359, -62.0218).. controls (37.6499, -61.8765) and (36.0995, -61.5588) .. (34.5871, -61.0576).. controls (34.0127, -60.8674) and (33.4468, -60.6541) .. (32.8925, -60.411).. controls (32.6755, -60.3157) and (32.4572, -60.2239) .. (32.2374, -60.1361).. controls (32.1479, -60.1004) and (32.0516, -60.0821) .. (31.9598, -60.0512).. controls (31.1851, -59.7892) and (30.3956, -59.5852) .. (29.5905, -59.4434).. controls (29.178, -59.3706) and (28.7629, -59.3159) .. (28.3453, -59.2783).. controls (27.9784, -59.2452) and (27.6109, -59.2286) .. (27.2426, -59.2233).. controls (26.8404, -59.2175) and (26.4385, -59.2296) .. (26.0379, -59.2648).. controls (24.7018, -59.382) and (23.4225, -59.7101) .. (22.2142, -60.3004).. controls (21.5344, -60.6324) and (20.9, -61.0357) .. (20.3094, -61.508).. controls (20.2732, -61.5371) and (20.2375, -61.5672) .. (20.1994, -61.5937).. controls (20.1681, -61.6154) and (20.1332, -61.6098) .. (20.1094, -61.5789).. controls (20.0118, -61.4521) and (19.9991, -61.4323) .. (20.1284, -61.3217).. controls (20.9037, -60.6589) and (21.599, -59.921) .. (22.206, -59.1008).. controls (22.6785, -58.4623) and (23.0828, -57.7842) .. (23.3871, -57.0484).. controls (23.5916, -56.5539) and (23.745, -56.0443) .. (23.8297, -55.5159).. controls (23.9125, -54.9997) and (23.9313, -54.4814) .. (23.8723, -53.9599).. controls (23.781, -53.1527) and (23.5215, -52.4028) .. (23.1188, -51.7009).. controls (22.5425, -50.6968) and (22.0504, -49.6536) .. (21.6479, -48.5682).. controls (21.2529, -47.503) and (20.9473, -46.4129) .. (20.7335, -45.2972).. controls (20.6404, -44.8109) and (20.5639, -44.3222) .. (20.5057, -43.8303).. controls (20.4425, -43.2964) and (20.401, -42.7609) .. (20.3769, -42.2238).. controls (20.3547, -41.7288) and (20.3528, -41.2337) .. (20.366, -40.7384).. controls (20.3774, -40.3196) and (20.4015, -39.901) .. (20.4404, -39.4838).. controls (20.6737, -36.9676) and (21.3397, -34.572) .. (22.4502, -32.3014).. controls (23.4304, -30.2961) and (24.7026, -28.4959) .. (26.258, -26.8954).. controls (26.7631, -26.3758) and (27.2947, -25.8852) .. (27.8498, -25.4198).. controls (28.0212, -25.2762) and (28.2107, -25.1701) .. (28.4305, -25.1206).. controls (29.1431, -24.9603) and (29.8783, -25.428) .. (30.0069, -26.1435).. controls (30.1006, -26.6652) and (29.9503, -27.1074) .. (29.5434, -27.4516).. controls (29.1068, -27.8209) and (28.683, -28.2038) .. (28.28, -28.6094).. controls (27.1547, -29.7421) and (26.198, -31.0028) .. (25.4098, -32.3911).. controls (24.624, -33.7751) and (24.0355, -35.2388) .. (23.6421, -36.7808).. controls (23.4976, -37.3467) and (23.3823, -37.9185) .. (23.2939, -38.4961).. controls (23.2362, -38.8726) and (23.187, -39.2501) .. (23.1537, -39.6296).. controls (23.1248, -39.9582) and (23.11, -40.2881) .. (23.0905, -40.6178).. controls (23.0664, -41.0279) and (23.0669, -41.4385) .. (23.0793, -41.8491).. controls (23.0915, -42.2468) and (23.1127, -42.6442) .. (23.1505, -43.0403).. controls (23.2119, -43.6851) and (23.3045, -44.3256) .. (23.4339, -44.9604).. controls (23.6953, -46.2418) and (24.0895, -47.4808) .. (24.6219, -48.6754).. controls (25.4852, -50.6121) and (26.6531, -52.3438) .. (28.1247, -53.8702).. controls (29.563, -55.3619) and (31.2092, -56.5724) .. (33.0631, -57.4987).. controls (34.4247, -58.179) and (35.8502, -58.6772) .. (37.3393, -58.9936).. controls (37.8029, -59.092) and (38.2696, -59.1735) .. (38.7392, -59.2349).. controls (39.1335, -59.2865) and (39.5293, -59.3246) .. (39.9267, -59.3495).. controls (40.4762, -59.3839) and (41.0258, -59.4008) .. (41.5764, -59.3841).. controls (41.991, -59.3717) and (42.4053, -59.3511) .. (42.8183, -59.3114).. controls (43.3025, -59.2648) and (43.7848, -59.2021) .. (44.2648, -59.1206).. controls (45.1673, -58.9674) and (46.0528, -58.7478) .. (46.9207, -58.4565).. controls (49.5025, -57.5897) and (51.7705, -56.2065) .. (53.7239, -54.3094).. controls (55.186, -52.8897) and (56.3682, -51.2643) .. (57.2754, -49.4395).. controls (57.8863, -48.2105) and (58.3464, -46.9273) .. (58.66, -45.5914).. controls (58.7925, -45.0268) and (58.8968, -44.4571) .. (58.9732, -43.8822).. controls (59.0275, -43.4753) and (59.0693, -43.0673) .. (59.0997, -42.6577).. controls (59.1439, -42.0619) and (59.1555, -41.4655) .. (59.1407, -40.8686).. controls (59.1315, -40.4963) and (59.114, -40.1241) .. (59.0743, -39.7536).. controls (59.0389, -39.4213) and (59.0071, -39.0885) .. (58.9611, -38.7575).. controls (58.8817, -38.1873) and (58.7708, -37.623) .. (58.6338, -37.0639).. controls (58.3269, -35.8103) and (57.8914, -34.6027) .. (57.3238, -33.4433).. controls (56.4986, -31.7574) and (55.436, -30.2371) .. (54.1388, -28.8806).. controls (53.5615, -28.2768) and (52.9452, -27.7162) .. (52.2893, -27.1992).. controls (52.1237, -27.0687) and (51.9861, -26.9161) .. (51.8917, -26.7274).. controls (51.4861, -25.917) and (51.9329, -24.9404) .. (52.8749, -24.7706).. controls (53.2638, -24.7004) and (53.6154, -24.7944) .. (53.9258, -25.0336).. controls (54.147, -25.2039) and (54.3626, -25.3823) .. (54.5748, -25.5638).. controls (56.6719, -27.3584) and (58.3525, -29.4828) .. (59.6088, -31.9408).. controls (60.4118, -33.5121) and (61.0015, -35.1607) .. (61.3788, -36.885).. controls (61.5045, -37.4597) and (61.6072, -38.0384) .. (61.6828, -38.6218).. controls (61.7389, -39.0541) and (61.7821, -39.4875) .. (61.8125, -39.9224).. controls (61.8461, -40.404) and (61.8617, -40.8861) .. (61.8688, -41.3689) -- cycle;

                                \path[fill=GemColorB] (38.2289, -22.8859) -- (38.2289, -22.8859).. controls (38.1056, -22.8859) and (38.0058, -22.9859) .. (38.0058, -23.1092).. controls (38.0058, -23.2325) and (38.1058, -23.3323) .. (38.2289, -23.3323) -- (38.2289, -23.3323).. controls (41.1554, -23.3323) and (43.5279, -25.7048) .. (43.5279, -28.6314) -- (43.5279, -28.6734).. controls (43.5279, -28.7967) and (43.6279, -28.8967) .. (43.751, -28.8967) -- (43.8354, -28.8967).. controls (43.9587, -28.8967) and (44.0584, -28.7967) .. (44.0584, -28.6734) -- (44.0584, -28.6314).. controls (44.0584, -25.7048) and (46.4309, -23.3323) .. (49.3575, -23.3323) -- (49.3575, -23.3323).. controls (49.4808, -23.3323) and (49.5805, -23.2323) .. (49.5805, -23.1092).. controls (49.5805, -22.9862) and (49.4805, -22.8859) .. (49.3575, -22.8859) -- (49.3575, -22.8859).. controls (46.4309, -22.8859) and (44.0584, -20.5134) .. (44.0584, -17.5869) -- (44.0584, -17.5448).. controls (44.0584, -17.4215) and (43.9584, -17.3215) .. (43.8354, -17.3215) -- (43.751, -17.3215).. controls (43.6277, -17.3215) and (43.5279, -17.4215) .. (43.5279, -17.5448) -- (43.5279, -17.5869).. controls (43.5279, -17.9091) and (43.4975, -18.2242) .. (43.4425, -18.5309).. controls (43.3062, -19.2876) and (43.0101, -19.9885) .. (42.5892, -20.5973).. controls (41.633, -21.9797) and (40.037, -22.8862) .. (38.2289, -22.8862) -- cycle;

                                \path[fill=GemColorA] (33.9468, -18.1917) -- (33.9468, -18.1917).. controls (33.8852, -18.1917) and (33.8352, -18.2417) .. (33.8352, -18.3033).. controls (33.8352, -18.365) and (33.8852, -18.415) .. (33.9468, -18.415) -- (33.9468, -18.415).. controls (35.4102, -18.415) and (36.5964, -19.6014) .. (36.5964, -21.0645) -- (36.5964, -21.0857).. controls (36.5964, -21.1474) and (36.6464, -21.1974) .. (36.708, -21.1974) -- (36.7501, -21.1974).. controls (36.8117, -21.1974) and (36.8618, -21.1474) .. (36.8618, -21.0857) -- (36.8618, -21.0645).. controls (36.8618, -19.6011) and (38.0481, -18.415) .. (39.5113, -18.415) -- (39.5113, -18.415).. controls (39.5729, -18.415) and (39.6229, -18.365) .. (39.6229, -18.3033).. controls (39.6229, -18.2417) and (39.5729, -18.1917) .. (39.5113, -18.1917) -- (39.5113, -18.1917).. controls (38.0479, -18.1917) and (36.8618, -17.0053) .. (36.8618, -15.5422) -- (36.8618, -15.521).. controls (36.8618, -15.4593) and (36.8117, -15.4093) .. (36.7501, -15.4093) -- (36.708, -15.4093).. controls (36.6464, -15.4093) and (36.5964, -15.4593) .. (36.5964, -15.521) -- (36.5964, -15.5422).. controls (36.5964, -15.7033) and (36.5813, -15.861) .. (36.5535, -16.0142).. controls (36.4855, -16.3925) and (36.3373, -16.7431) .. (36.127, -17.0474).. controls (35.6489, -17.7387) and (34.8509, -18.1917) .. (33.9468, -18.1917) -- cycle;

                                \path[fill=GemColorC] (33.3158, -25.9583) -- (33.3158, -25.9583).. controls (33.2788, -25.9583) and (33.2486, -25.9884) .. (33.2486, -26.0255).. controls (33.2486, -26.0625) and (33.2788, -26.0927) .. (33.3158, -26.0927) -- (33.3158, -26.0927).. controls (34.1958, -26.0927) and (34.9091, -26.806) .. (34.9091, -27.686) -- (34.9091, -27.6987).. controls (34.9091, -27.7357) and (34.9393, -27.7659) .. (34.9763, -27.7659) -- (35.0017, -27.7659).. controls (35.0388, -27.7659) and (35.0689, -27.7357) .. (35.0689, -27.6987) -- (35.0689, -27.686).. controls (35.0689, -26.806) and (35.7823, -26.0927) .. (36.6623, -26.0927) -- (36.6623, -26.0927).. controls (36.6993, -26.0927) and (36.7295, -26.0625) .. (36.7295, -26.0255).. controls (36.7295, -25.9884) and (36.6993, -25.9583) .. (36.6623, -25.9583) -- (36.6623, -25.9583).. controls (35.7823, -25.9583) and (35.0689, -25.245) .. (35.0689, -24.365) -- (35.0689, -24.3522).. controls (35.0689, -24.3152) and (35.0388, -24.285) .. (35.0017, -24.285) -- (34.9763, -24.285).. controls (34.9393, -24.285) and (34.9091, -24.3152) .. (34.9091, -24.3522) -- (34.9091, -24.365).. controls (34.9091, -24.4618) and (34.8999, -24.5565) .. (34.8835, -24.6488).. controls (34.8425, -24.8764) and (34.7536, -25.0873) .. (34.6268, -25.2701).. controls (34.3392, -25.6858) and (33.8595, -25.9583) .. (33.3158, -25.9583) -- cycle;

                                % Centered bold sans-serif "AI" (now at the origin)
                                \node[anchor=center, font=\llmIconAIFont, color=\llmIconAIColor] at (40.5, -41) {AI};

                            \end{scope}
                        \end{scope}
                    \end{scope}
                }}
}


==> new_plots/init_plot/pipeline_overview_vertical.tex <==
% Pipeline overview diagram composed from existing fragments
% - Uses example env thumbnails from example_envs.tex in the selector box
% - Uses prebuilt PDF of the interaction fragment (interaction_phase_preview.pdf)
% - Uses separate test phase fragment from test_phase.tex
% This file is a fragment intended to be \subimport'ed or \input into a figure/tikzpicture
% Example standalone preview provided in pipeline_overview_preview.tex

% Dependencies: \usepackage{tikz}, \usepackage{import}
\usetikzlibrary{arrows.meta,calc,shapes.callouts}

\providecommand{\pipelineArrowHeadLength}{3mm}
\providecommand{\pipelineArrowHeadWidth}{2.2mm}
\providecommand{\ipArrowHeadLength}{3mm}
\providecommand{\ipArrowHeadWidth}{2.2mm}
\providecommand{\ipLabelFont}{\normalsize}
\providecommand{\pipelineSectionTitleFont}{\small\bfseries}
\providecommand{\pipelineSectionTitleYOffset}{0.2cm}
\providecommand{\pipelineSectionFrameLineWidth}{0.8pt}
\providecommand{\pipelineSectionFrameCorner}{6pt}
\providecommand{\pipelineSectionPadX}{0.15cm}
\providecommand{\pipelineSectionPadYBottom}{0.05cm}
\providecommand{\pipelineSectionPadYTop}{0.0cm}
\providecommand{\pipelineTestPhaseXShift}{4.2cm}
\providecommand{\pipelineTestPhaseScale}{0.95}
\providecommand{\pipelineAgentLabelYOffset}{0.40cm}
\providecommand{\pipelineActorArrowXOffset}{1.3}
\providecommand{\pipelineArrowLabelFill}{labelBg}

% Styles - Updated to match interaction phase format
\tikzset{
% Match interaction phase arrow style exactly
pipeline/arrow/.style={draw=black, line width=1pt, line cap=round, line join=round, -{Stealth[length=\pipelineArrowHeadLength,width=\pipelineArrowHeadWidth]}, shorten <=1.6mm, shorten >=1.6mm, preaction={draw=white, line width=2.2pt, opacity=0.9}},
pipeline/label/.style={font=\normalsize, text=black},
pipeline/descbox/.style={rounded corners=2pt, draw=none, inner sep=2pt, text width=3.2cm, align=left}
}

% Colors for task description boxes
\colorlet{CDColor}{cyan!18}
\colorlet{PLColor}{orange!20}
\colorlet{MFPColor}{green!20}
% Lavender color for agent box
\definecolor{lavender}{RGB}{230, 230, 250}
\definecolor{lightbulb}{RGB}{255,235,59}

% Unified thumbnail height for task grids (smaller & equal-sized)
\newcommand{\TaskThumbH}{3cm}

% Provide defaults required by the grid fragments
\providecommand{\maraGridLineColor}{black!10}
\providecommand{\maraGridBorderColor}{black!30}
\providecommand{\maraGridLineWidth}{0.4pt}
\providecommand{\maraBorderLineWidth}{3pt}
\providecommand{\maraBorderRadius}{2pt}

% Default label background
\providecolor{labelBg}{HTML}{F7F4EE}

% Coordinate system (units: cm)
\begin{scope}[x=1cm,y=1cm]

  % Padding for the example envs dashed box. The envs container is shifted down
  % by \pipelineEnvTopShift so the dashed border doesn't hug the grids while
  % the title still aligns with "Test Phase" in y.
  % Match the horizontal padding of the interaction-phase box so the two
  % dashed boxes can share the exact same left x coordinate.
  \providecommand{\pipelineEnvSectionPadX}{\pipelineSectionPadX}
  \providecommand{\pipelineEnvSectionPadYBottom}{0.05cm}
  \providecommand{\pipelineEnvSectionPadYTop}{0.15cm}
  \providecommand{\pipelineEnvTopShift}{0.15cm}

  % Test phase (right) - rendered first so its top can anchor the example envs row
  \begin{scope}[shift={(\pipelineTestPhaseXShift,0)}, scale=\pipelineTestPhaseScale, local bounding box=tpbb]
    % \clip (0,0) rectangle (6cm, 10cm);
    \subimport{.}{test_phase_vertical.tex}
  \end{scope}

  % Enclose the test phase with a dashed line box
  \draw[dashed, line width=\pipelineSectionFrameLineWidth, rounded corners=\pipelineSectionFrameCorner]
  ([xshift=-\pipelineSectionPadX,yshift=-\pipelineSectionPadYBottom]tpbb.south west)
  rectangle
  ([xshift=\pipelineSectionPadX,yshift=\pipelineSectionPadYTop]tpbb.north east);

  % Label above the test phase
  \node[pipeline/label, font=\pipelineSectionTitleFont]
  at ([yshift=\pipelineSectionTitleYOffset]tpbb.north) {Test Phase};

  % Interaction elements (left) - rendered before the envs container so we can
  % anchor the envs dashed box left edge to ipbb.west for x-alignment.
  \begin{scope}[shift={(0,-0.3)}, scale=0.9, local bounding box=ipbb]
    \subimport{.}{interaction_phase.tex}
  \end{scope}

  % Enclose the interaction phase with a dashed line box
  \draw[dashed, line width=\pipelineSectionFrameLineWidth, rounded corners=\pipelineSectionFrameCorner]
  ([xshift=-\pipelineSectionPadX,yshift=-\pipelineSectionPadYTop]ipbb.south west)
  rectangle
  ([xshift=\pipelineSectionPadX,yshift=\pipelineSectionPadYTop]ipbb.north east);

  % Select env thumbnails (top-left). Wrap the imported scope in a node so its
  % top can be anchored at the same y as the test phase's top, and its dashed
  % box left aligned with the interaction phase dashed box left.
  \node[anchor=north west, inner sep=0pt] (envscontainer)
    at ([yshift=-\pipelineEnvTopShift]ipbb.west |- tpbb.north) {%
    \begin{tikzpicture}
      % Local override: more breathing room between each grid and its caption.
      % poster.tex defines this globally, so use \renewcommand (group-local).
      \renewcommand{\maraCaptionGap}{0.3cm}
      \begin{scope}[scale=0.46, local bounding box=exbb]
        \subimport{.}{example_envs.tex}
      \end{scope}
    \end{tikzpicture}%
  };
  % Enclose the example environments with a dashed line box. Left edge is taken
  % directly from ipbb's dashed box so the two left edges coincide.
  \draw[dashed, line width=\pipelineSectionFrameLineWidth, rounded corners=\pipelineSectionFrameCorner]
  ([xshift=-\pipelineEnvSectionPadX,yshift=-\pipelineEnvSectionPadYBottom]envscontainer.south west)
  rectangle
  ([xshift=\pipelineEnvSectionPadX,yshift=\pipelineEnvSectionPadYTop]envscontainer.north east);
  % Label above the example envs block (same y as the Test Phase title:
  % envscontainer.north sits \pipelineEnvTopShift below tpbb.north, so we
  % add that back here so the title lands at tpbb.north + \pipelineSectionTitleYOffset)
  \node[pipeline/label, font=\pipelineSectionTitleFont]
  at ([yshift=\pipelineSectionTitleYOffset+\pipelineEnvTopShift]envscontainer.north) {AutumnBench Environments};

  % Label above the interaction phase
  \node[pipeline/label, font=\pipelineSectionTitleFont]
  at ([yshift=\pipelineSectionTitleYOffset]ipbb.north) {Interaction Phase};

  % (Yellow callout notes removed for poster use.)
  \coordinate (betweenPhasesMid) at ($ (ipbb.east)!0.5!(tpbb.west) $);

  % Ensure interaction-phase styles/colors exist outside the imported scope
  \tikzset{
  ip/box/.style={draw, rounded corners=6pt, minimum width=4.2cm, minimum height=3.0cm, line width=0.8pt, align=center, font=\large},
  ip/arrow/.style={line width=1pt, line cap=round, line join=round, -{Stealth[length=\ipArrowHeadLength,width=\ipArrowHeadWidth]}, shorten <=1.6mm, shorten >=1.6mm, preaction={draw=white, line width=2.2pt, opacity=0.9}},
  ip/label/.style={font=\ipLabelFont, fill=labelBg, inner sep=2pt, rounded corners=2pt}
  }
  \colorlet{IPRightBg}{red!30!brown!35}

  % Explorer/agent interaction loop (moved from interaction_phase)
  % Two actor icons (LLM or Human) with an "OR" between them
  % Positioned near previous agent location
  % Background containers (used for fitting and arrow anchors) - moved higher
  \begin{scope}[shift={(0,-0.2)}]
    \node[rounded corners=12pt, minimum width=1.0cm, minimum height=.8cm, draw=none] (llm) at (1.4,.6) {};
    \node[rounded corners=12pt, minimum width=1.0cm, minimum height=.8cm, draw=none] (human) at (3.0,.6) {};

    % Fit node around both actors to anchor arrows
    \node[inner sep=1pt, fit=(llm) (human)] (actors) {};

    % LLM robot icon via pic (drawn on top of background)
    \subimport{.}{pic_llm_icon.tex}
    \pic[scale=0.02] at (llm.center) {llm_icon};

    % Human icon via pic (drawn on top of background)
    \subimport{.}{pic_human_icon.tex}
    \pic[scale=0.05] at (human.center) {human_icon};

    % Agents dashed box enclosing both icons (narrower horizontally)
    \draw[dashed, line width=\pipelineSectionFrameLineWidth, rounded corners=\pipelineSectionFrameCorner]
    ([xshift=-0.05cm,yshift=-0.2cm]actors.south west)
    rectangle
    ([xshift= 0.05cm,yshift= 0.2cm]actors.north east);
    % Label above the agents box.
    \node[pipeline/label, font=\pipelineSectionTitleFont]
    at ([yshift=\pipelineAgentLabelYOffset]actors.north) {Agent};

    % OR separator: slashed line with label above
    \draw[draw=black, line width=0.9pt] (2.05,0.25) -- (2.35,0.95);

    % CURVED arrow system between boxes
    % Get the actual bounds of the stack and actors boxes
    \coordinate (stackBottom) at ($ (stack.south) + (0,-0.5) $);
    \coordinate (agentTop) at (actors.north);

    % Horizontal offsets for the two arrow columns from the center
    \def\ArrowXOffset{\pipelineActorArrowXOffset}

    % State arrow (left side): Environment state flows DOWN to agent - CURVED
    \draw[ip/arrow]
    ($ (stackBottom)+(-\ArrowXOffset + 0.2, 0) $)
    .. controls +(-0.4, -0.3) and +(-0.4, 0.5) ..
    coordinate[pos=0.5] (obsMid)
    ($ (agentTop)+(-\ArrowXOffset, 0) $);
    \node[ip/label, fill=\pipelineArrowLabelFill, text=black] at (obsMid) {observation};

    % Action arrow (right side): Agent actions flow UP to environment - CURVED
    \draw[ip/arrow]
    ($ (agentTop)+(\ArrowXOffset, 0) $)
    .. controls +(0.4, 0.3) and +(0.1, -0.3) ..
    coordinate[pos=0.5] (actMid)
    ($ (stackBottom)+(\ArrowXOffset, 0) $);
    \node[ip/label, fill=\pipelineArrowLabelFill, text=black] at (actMid) {action};

    % Arrows connecting the pipeline phases
    % Arrow from examples to interaction phase with broken line and label in the break
    \def\arrowOneStartX{1.8}
    \def\arrowOneStartY{6.8}
    \coordinate (ip-north) at (ipbb.north);
    \def\arrowOneLabelY{6.1} % midpoint for label placement

    % First part of arrow (before break)
    % \draw[pipeline/arrow, -] (\arrowOneStartX, \arrowOneStartY) -- (\arrowOneStartX, {\arrowOneLabelY+0.05});
    % Label at the break (matching interaction phase label style)
    % \node[font=\tiny, text=black] at (\arrowOneStartX, \arrowOneLabelY) {select environment};
    % Second part of arrow (after break, with arrowhead)
    % \draw[pipeline/arrow] (\arrowOneStartX, {\arrowOneLabelY-0.05}) -- (ip-north);

    % % Arrow from interaction phase to test phase  
    % \draw[pipeline/arrow] (ipbb.east) -- (tpbb.west);

    % Also draw observation/action arrows between actors and the test phase
    % Define convenient anchors (offset so start/end points differ)
    \coordinate (actorsRight) at (actors.east);
    \coordinate (actorsObs) at ($ (actorsRight)+(0, 0.25) $);
    \coordinate (actorsAct) at ($ (actorsRight)+(0,-0.25) $);
    % Project test-phase west edge to the same y-levels as actors for horizontal arrows
    \coordinate (testObs) at ($ (tpbb.west |- actorsObs) $);
    \coordinate (testAct) at ($ (tpbb.west |- actorsAct) $);

    % Observation (from test phase to actors) - arched upward
    \draw[ip/arrow]
    (testObs)
    .. controls +(-0.6, 0.6) and +(0.6, 0.6) ..
    coordinate[pos=0.5] (phaseObsMid)
    (actorsObs);
    \node[ip/label, fill=\pipelineArrowLabelFill, text=black] at (phaseObsMid) {observation};

    % Action (from actors to test phase) - arched downward
    \draw[ip/arrow]
    (actorsAct)
    .. controls +(0.6, -0.6) and +(-0.6, -0.6) ..
    coordinate[pos=0.5] (phaseActMid)
    (testAct);
    \node[ip/label, fill=\pipelineArrowLabelFill, text=black] at (phaseActMid) {action};
  \end{scope}

\end{scope}


==> new_plots/init_plot/stacked_treasure.tex <==
% Stacked figure using diagrams/treasure.tikz as a sub-figure
% This is a fragment intended to be \subimport'ed into a tikzpicture or figure
% Usage example (standalone preview provided in stacked_treasure_preview.tex):
% \begin{tikzpicture}
%   \subimport{.}{stacked_treasure.tex}
% \end{tikzpicture}

% Requires: \usepackage{import}

% Provide defaults for MARA grid style if not already defined
\providecommand{\maraGridLineColor}{black!10}
\providecommand{\maraGridBorderColor}{black!30}
\providecommand{\maraGridLineWidth}{0.4pt}
\providecommand{\maraBorderLineWidth}{3pt}
\providecommand{\maraBorderRadius}{2pt}

% Overlay three copies diagonally to match the reference look
\begin{scope}
  % back (top-left)
  \begin{scope}[shift={(-0.3,0.6)}]
    \subimport{../../diagrams/}{treasure_single_1.tikz}
  \end{scope}
  % middle
  \begin{scope}[shift={(0.0,0.3)}]
    \subimport{../../diagrams/}{treasure_single_2.tikz}
  \end{scope}
  % front (bottom-right)
  \begin{scope}[shift={(0.3,0.0)}]
    \subimport{../../diagrams/}{treasure_single_3.tikz}
  \end{scope}
\end{scope}




==> new_plots/init_plot/test_phase.tex <==
% Test phase fragment: three task rows (CD, PL, MFP) with thumbnails
% Intended to be \subimport'ed into a parent tikzpicture
% Assumes parent sets [x=1cm,y=1cm] (coordinates in cm)
% Requires: \usepackage{graphicx}, \usepackage{import}, \usetikzlibrary{positioning,fit}
% Local load for wavy arrow decoration
\usetikzlibrary{decorations.pathmorphing}

% Default sizes if not provided by parent
\providecommand{\TaskThumbH}{3cm}
\providecommand{\TaskRowW}{3.2cm}
\providecommand{\TaskRowSep}{0.4cm}   % vertical spacing between task rows
% Browser header configuration
\providecommand{\BrowserBarH}{0.5cm} % adjustable title bar height
\providecommand{\BrowserBarAddrTop}{0.12cm}
\providecommand{\BrowserBarAddrBottomPad}{0.12cm}
% Local styles for task name boxes
\colorlet{TaskCDColor}{cyan!18}
\colorlet{TaskPLColor}{orange!20}
\colorlet{TaskMFPColor}{green!20}

\tikzset{task/namebox/.style={draw=none, rounded corners=12pt, font=\small, text=black, align=center, inner sep=6pt, minimum height=\TaskThumbH, minimum width=3.0cm}}
\tikzset{task/content/.style={inner sep=0, anchor=west}}
\tikzset{task/row/.style={inner sep=0, anchor=north west}}

% Styles for the enclosing box and title
\tikzset{task/outerbox/.style={draw=black, rounded corners=8pt, line width=0.8pt}}
\tikzset{task/title/.style={font=\large\bfseries, text=black}}
% Style for per-row captions
\tikzset{task/caption/.style={font=\scriptsize, text=black}}

% Style for CD arrow
\tikzset{cd/arrow/.style={decorate, decoration={snake, amplitude=0.3mm, segment length=2mm, pre length=0.6mm, post length=3mm}, -{Stealth[length=1.5mm,width=1.2mm]}, shorten >=1.6mm, line cap=round, line width=0.6pt, color=gray}}

\begin{scope}[node distance=\TaskRowSep]
  % Place each pic as the content of a node so positioning works horizontally
  % Tasks arranged left-to-right: MFP | PL | CD
  % All aligned to y=0 baseline using projection (|- 0,0)

  % MFP column (leftmost)
  % Backdrop center aligns at parent y = 1.75 cm (file center 5*0.35 cm with outer y=0).
  \begin{scope}[shift={(0,0cm)}]
    \begin{scope}[local bounding box=MFPbb]
      \subimport{.}{mfp_example.tex}
    \end{scope}
    \node[inner sep=0, outer sep=0, fit=(MFPbb)] (MFPRow) {};
  \end{scope}

  % PL column (middle) - backdrop center already at 1.75 cm with outer y=0.
  \begin{scope}[shift={($(MFPbb.east |- 0,0)+(0.5cm,0cm)$)}]
    \begin{scope}[local bounding box=PLbb]
      \subimport{.}{planning_example.tex}
    \end{scope}
    \node[inner sep=0, outer sep=0, fit=(PLbb)] (PLRow) {};
  \end{scope}

  % CD column - CD1 backdrop center at file y=6.2 cellsz (=2.17 cm); shift down by -0.42 cm to match 1.75 cm.
  \begin{scope}[local bounding box=CDbb]
    \begin{scope}[shift={($(PLbb.east |- 0,0)+(0.5cm,-0.42cm)$)}]
      \begin{scope}[local bounding box=CD1bb]
        \subimport{.}{cd_example.tex}
      \end{scope}
      \node[inner sep=0, outer sep=0, fit=(CD1bb)] (CD1Row) {};
    \end{scope}

    % Second CD panel - backdrop center at file y=5.65 cellsz; shift -0.228 cm to align center at 1.75 cm.
    \begin{scope}[shift={($(CD1bb.east |- 0,0)+(0.5cm,-0.2275cm)$)}]
      \begin{scope}[local bounding box=CD2bb]
        \subimport{.}{cd_example_slider.tex}
      \end{scope}
      \node[inner sep=0, outer sep=0, fit=(CD2bb)] (CD2Row) {};
    \end{scope}

    % Arrow between the two CD panels
    \draw[cd/arrow] ([xshift=-0.20cm]CD1Row.east) -- ([xshift=0.25cm]CD2Row.west |- CD1Row.east);
  \end{scope}
  \node[inner sep=0, outer sep=0, fit=(CDbb)] (CDRow) {};

  % Overall content bounding box for separator lines
  \node[inner sep=0, outer sep=0, fit=(CDRow) (PLRow) (MFPRow)] (contentfit) {};

  % Vertical separators between task kinds
  \coordinate (sepMFPPL) at ($(MFPbb.east)!0.5!(PLbb.west)$);
  \coordinate (sepPLCD) at ($(PLbb.east)!0.5!(CDbb.west)$);
  \draw[color=gray!55, line width=0.5pt]
  (contentfit.north -| sepMFPPL) -- ([yshift=-0.5cm]contentfit.south -| sepMFPPL);
  \draw[color=gray!55, line width=0.5pt]
  (contentfit.north -| sepPLCD) -- ([yshift=-0.5cm]contentfit.south -| sepPLCD);

  % Captions below each task column - aligned to the lowest row south
  \node[inner sep=0, outer sep=0, fit=(MFPRow)(PLRow)(CDRow)] (AllRows) {};
  \node[task/caption, anchor=north] at ($(AllRows.south -| MFPRow)+(0,-0.1cm)$) {Masked Frame Prediction};
  \node[task/caption, anchor=north] at ($(AllRows.south -| PLRow)+(0,-0.1cm)$) {Planning};
  \node[task/caption, anchor=north] at ($(AllRows.south -| CDRow)+(0,-0.1cm)$) {Change Detection};
  % % Outer frame
  % \node[
  %   draw=black, line width=0.8pt, rounded corners=8pt, inner sep=1em,
  %   fit=(CDRow) (PLRow) (MFPRow)
  % ] {};
  % % Draw the enclosing box with asymmetric padding
  % \draw[task/outerbox]
  % ([shift={(-\TaskBoxPadX,-\TaskBoxPadYBottom)}]contentfit.south west)
  % rectangle
  % ([shift={(\TaskBoxPadX,\TaskBoxPadYTop)}]contentfit.north east);
\end{scope}

==> new_plots/init_plot/test_phase_vertical.tex <==
% Test phase fragment: three task rows (CD, PL, MFP) with thumbnails
% Intended to be \subimport'ed into a parent tikzpicture
% Assumes parent sets [x=1cm,y=1cm] (coordinates in cm)
% Requires: \usepackage{graphicx}, \usepackage{import}, \usetikzlibrary{positioning,fit}
% Local load for wavy arrow decoration
\usetikzlibrary{decorations.pathmorphing}

% Default sizes if not provided by parent
\providecommand{\TaskThumbH}{3cm}
\providecommand{\TaskRowW}{3.2cm}
\providecommand{\TaskRowSep}{0.9cm}   % vertical spacing between task rows
% Browser header configuration
\providecommand{\BrowserBarH}{0.5cm} % adjustable title bar height
\providecommand{\BrowserBarAddrTop}{0.12cm}
\providecommand{\BrowserBarAddrBottomPad}{0.12cm}
\providecommand{\cdArrowHeadLength}{1.5mm}
\providecommand{\cdArrowHeadWidth}{1.2mm}
\providecommand{\cdArrowAmplitude}{0.3mm}
\providecommand{\cdArrowSegmentLength}{2mm}
\providecommand{\cdArrowPreLength}{0.6mm}
\providecommand{\cdArrowPostLength}{3mm}
\providecommand{\cdArrowLineWidth}{0.6pt}
\providecommand{\TaskCaptionFont}{\scriptsize}
\providecommand{\TaskCaptionYOffset}{-0.1cm}
% NOTE: do NOT override \TaskInnerTitle* here; each subimported file already
% provides its own \providecommand defaults that match its standalone layout.
% Overriding them in the parent pushes titles off their natural positions
% (and causes the "Reach the target configuration:" / "Interact until detect
% change:" text overflow).
\providecommand{\TaskCDPanelGap}{3.0cm}
\providecommand{\TaskSingleRowXOffset}{1.5cm}
% Horizontal offset from a row's content origin (lower-left of backdrop)
% to the visual center of that row's bounding box. Used to center each row
% on CDbb's center. Defaults derived from backdrop widths in each file.
\providecommand{\TaskPLCenterOffset}{2.55cm}   % planning_example: 14.6 cells * 0.35cm / 2
\providecommand{\TaskMFPCenterOffset}{2.45cm}  % mfp_example: 14 cells * 0.35cm / 2
% Local styles for task name boxes
\colorlet{TaskCDColor}{cyan!18}
\colorlet{TaskPLColor}{orange!20}
\colorlet{TaskMFPColor}{green!20}

\tikzset{task/namebox/.style={draw=none, rounded corners=12pt, font=\small, text=black, align=center, inner sep=6pt, minimum height=\TaskThumbH, minimum width=3.0cm}}
\tikzset{task/content/.style={inner sep=0, anchor=west}}
\tikzset{task/row/.style={inner sep=0, anchor=north west}}

% Styles for the enclosing box and title
\tikzset{task/outerbox/.style={draw=black, rounded corners=8pt, line width=0.8pt}}
\tikzset{task/title/.style={font=\large\bfseries, text=black}}
% Style for per-row captions
\tikzset{task/caption/.style={font=\TaskCaptionFont, text=black}}

% Style for CD arrow
\tikzset{cd/arrow/.style={decorate, decoration={snake, amplitude=\cdArrowAmplitude, segment length=\cdArrowSegmentLength, pre length=\cdArrowPreLength, post length=\cdArrowPostLength}, -{Stealth[length=\cdArrowHeadLength,width=\cdArrowHeadWidth]}, shorten >=1.6mm, line cap=round, line width=\cdArrowLineWidth, color=gray}}

\begin{scope}[node distance=\TaskRowSep]
  % CD row at the bottom (anchor for centering the others)
  \begin{scope}[local bounding box=CDbb]
    % First CD panel
    \begin{scope}[shift={(1.5,0)}]
      \begin{scope}[local bounding box=CD1bb]
        \subimport{.}{cd_example.tex}
      \end{scope}
      \node[inner sep=0, outer sep=0, fit=(CD1bb)] (CD1Row) {};
    \end{scope}

    % Second CD panel
    \begin{scope}[shift={({1.5cm+\TaskCDPanelGap},0)}]
      \begin{scope}[local bounding box=CD2bb]
        \subimport{.}{cd_example_slider.tex}
      \end{scope}
      \node[inner sep=0, outer sep=0, fit=(CD2bb)] (CD2Row) {};
    \end{scope}

    % Arrow between the two CD panels: span the full inter-panel gap.
    \draw[cd/arrow] ([xshift=-0.20cm]CD1Row.east) -- ([xshift=0.25cm]CD2Row.west |- CD1Row.east);
  \end{scope}
  \node[inner sep=0, outer sep=0, fit=(CDbb)] (CDRow) {};

  % PL row above CD. Direct subimport (so the parent's scale propagates).
  % Shift puts PL's content origin (its backdrop's lower-left) at
  % x = CDbb.center.x - \TaskPLCenterOffset, y = CDbb.north.y + \TaskRowSep,
  % which centers PL's bbox horizontally on CDbb's center.
  \begin{scope}[shift={($(CDbb.center |- CDbb.north)+(-\TaskPLCenterOffset,\TaskRowSep)$)}]
    \begin{scope}[local bounding box=PLbb]
      \subimport{.}{planning_example.tex}
    \end{scope}
    \node[inner sep=0, outer sep=0, fit=(PLbb)] (PLRow) {};
  \end{scope}

  % MFP row above PL, centered on the same vertical axis as CDbb.
  \begin{scope}[shift={($(CDbb.center |- PLbb.north)+(-\TaskMFPCenterOffset,\TaskRowSep)$)}]
    \begin{scope}[local bounding box=MFPbb]
      \subimport{.}{mfp_example.tex}
    \end{scope}
    \node[inner sep=0, outer sep=0, fit=(MFPbb)] (MFPRow) {};
  \end{scope}

  % Captions sit just below each row's south edge — drawn FIRST so the
  % dividers can be placed below the captions (caption above divider).
  \node[task/caption, anchor=north] (capMFP) at ($(MFPRow.south)+(0,\TaskCaptionYOffset)$) {Masked Frame Prediction};
  \node[task/caption, anchor=north] (capPL)  at ($(PLRow.south)+(0,\TaskCaptionYOffset)$) {Planning};
  \node[task/caption, anchor=north] (capCD)  at ($(CDRow.south)+(0,\TaskCaptionYOffset)$) {Change Detection};

  % Overall content bounding box for separator lines (excluding captions/dividers)
  \node[inner sep=0, outer sep=0, fit=(CDRow) (PLRow) (MFPRow)] (contentfit) {};

  % Horizontal separators: placed BELOW each caption so the caption sits
  % above the divider and stays grouped with its row.
  \coordinate (sepPLMFP) at ($(capMFP.south)!0.5!(PLRow.north)$);
  \coordinate (sepCDPL)  at ($(capPL.south)!0.5!(CDRow.north)$);
  \draw[color=gray!55, line width=0.5pt]
    (contentfit.west |- sepPLMFP) -- (contentfit.east |- sepPLMFP);
  \draw[color=gray!55, line width=0.5pt]
    (contentfit.west |- sepCDPL) -- (contentfit.east |- sepCDPL);
  % % Outer frame
  % \node[
  %   draw=black, line width=0.8pt, rounded corners=8pt, inner sep=1em,
  %   fit=(CDRow) (PLRow) (MFPRow)
  % ] {};
  % % Draw the enclosing box with asymmetric padding
  % \draw[task/outerbox]
  % ([shift={(-\TaskBoxPadX,-\TaskBoxPadYBottom)}]contentfit.south west)
  % rectangle
  % ([shift={(\TaskBoxPadX,\TaskBoxPadYTop)}]contentfit.north east);
\end{scope}

